Mismatch Quest: Visual and Textual Feedback for Image-Text Misalignment

While existing image-text alignment models reach high quality binary assessments, they fall short of pinpointing the exact source of misalignment. In this paper, we present a method to provide detailed textual and visual explanation of detected misalignments between text-image pairs. We leverage large language models and visual grounding models to automatically construct a training set that holds plausible misaligned captions for a given image and corresponding textual explanations and visual indicators. We also publish a new human curated test set comprising ground-truth textual and visual misalignment annotations. Empirical results show that fine-tuning vision language models on our training set enables them to articulate misalignments and visually indicate them within images, outperforming strong baselines both on the binary alignment classification and the explanation generation tasks. Our method code and human curated test set are available at: https://mismatch-quest.github.io/

==> figures/nli_premise_hypo.tex <==
\begin{figure}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}
    \node[draw, rounded corners, fill=blue!10, align=left, text width=\columnwidth, inner sep=5pt, font=\scriptsize] {
    \underline{\textbf{Feedback Evaluation Task}}: \\
    \textbf{Contradiction Correctness:} \\
    \textbf{Premise:} \textit{Positive Caption: \poscaption} \\
    \textbf{Hypothesis:} \textit{Generated Contradiction: \negcaption} \\
    \textbf{Entailment Score:} 0.12 (Low) \\
    \textbf{Feedback Correctness:} \\
    \textbf{Premise:} \textit{Positive Caption: \poscaption\ Negative Caption: \negcaption} \\
    \textbf{Hypothesis:} \textit{Feedback: \feedbacktext} \\
    \textbf{Entailment Score:} 0.91 (High) \\
    };
\end{tikzpicture}%
}
\caption{Feedback evaluation using NLI models, indicated by entailment scores for contradiction and feedback generation.}
\label{fig:feedback_evaluation}
\end{figure}

==> images/prompts/ade20k_attribute.tex <==
\begin{figure*}
\centering
\footnotesize
\begin{tabular}{p{\linewidth}}
\toprule
Context \\
\midrule
Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.\\
\\
Guidelines:\\
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:\\
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").\\
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").\\
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\


\midrule
Few-Shot \\
\midrule

Guidelines:\\
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.\\
\\
Examples: \\
\\
CAPTION: "a waterfall in a tropical forest with green plants and trees"\\
CONTRADICTION: a waterfall in a snowy forest with green plants and trees\\
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)\\
MISALIGNMENT TYPE: Attribute/Adjective\\
\\
CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"\\
CONTRADICTION: a cartoon of a mermaid with black hair in the water\\
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with black hair)\\
MISALIGNMENT TYPE: Attribute/Adjective\\
\\
CAPTION: portrait of a naked woman with long hair on a grey background\\
CONTRADICTION: A portrait of a naked woman with short hair on a grey background\\
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)\\
MISALIGNMENT TYPE: Attribute/Adjective\\
\\
CAPTION: The colorful flowers are in the vase next to the window.\\
CONTRADICTION: The white and black flowers are in the vase next to the window.\\
MISALIGNMENT: The flowers are colorful (CAPTION: colorful flowers) , not white and black (CONTRADICTION: white and black flowers)\\
MISALIGNMENT TYPE: Attribute/Adjective\\
\\
CAPTION: Vase sitting next to the window with droopy flowers in it.\\
CONTRADICTION: Vase sitting next to the window with fresh flowers in it.\\
MISALIGNMENT: The vase has droppy flowers (CAPTION: droppy flowers), not fresh flowers (CAPTION: fresh flowers)\\
MISALIGNMENT TYPE: Attribute/Adjective\\
\\
CAPTION: A bicycle chained to a red pole and a green pole on the sidewalk in front of a building.\\
CONTRADICTION: A bicycle chained to a red pole and a blue pole on the sidewalk in front of a building.\\
MISALIGNMENT: One of the poles is red (CAPTION: green pole), not blue (CONTRADICTION: blue pole)\\
MISALIGNMENT TYPE: Attribute/Adjective\\
\\
Create a MISALIGNMENT of type: Attribute/Adjective\\
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.\\
CAPTION: A wall with light and dust particles under a wooden beam. \\

\midrule
Generated \\
\midrule
CONTRADICTION: A wall with light and dust particles under a metal beam.\\
MISALIGNMENT: The beam is wood (CAPTION: wooden beam), not metal (CONTRADICTION: metal beam)\\
MISALIGNMENT TYPE: Attribute/Adjective\\
\bottomrule
\end{tabular}   
\caption{Few-shot prompt example for generating an \emph{Attribute} misalignment in the ADE20k~\cite{ade20k_zhou2017scene} dataset.}
\label{fig:prompt_ade20k_noun}

\end{figure*}


==> images/prompts/ade20k_description_to_caption.tex <==
\begin{figure*}
\centering
\footnotesize
\begin{tabular}{p{\linewidth}}
\toprule
Context \\
\midrule

Task Definition: Extracting Concise Image Captions\\
\\
Input: \\
DESCRIPTION: A long description of an image containing various objects, people, and scene details.\\
\\
Output: \\
CAPTION: A single-sentence caption that preserve all the information from the description.\\
\\
Guidelines:\\
- The goal is to create a concise caption that effectively communicates the image's information written as a caption not a description.\\
- Include what people are doing and wearing from the description.\\
- Describe where objects are and how they look from the description.\\

\midrule
Few-Shot \\
\midrule

Examples:\\
\\
DESCRIPTION: Front we can see ball. Background it is blur. We can see trees, people and sky.\\
CAPTION: A ball with a blur background that includes trees, people and sky\\
\\
DESCRIPTION: There is a poster in which, there is a image. In the image, there are two vehicles parked on the grass on the ground. In the background, there are trees. Below this image, there are texts and watermark on the white page. \\
CAPTION: An image of two vehicles parked on the grass, below the image there is a text.\\
\\
DESCRIPTION: In this picture I can see food items, fork and a bowl with a liquid in it, on the plate, on an object.\\
CAPTION: Food items, fork and a bowl with liquid in it are on a plate.\\
\\
DESCRIPTION: This image is taken outdoors. At the top of the image there is the sky. At the bottom of the image there is a runway. In the background there are a few buildings and there is a ground with grass on it. In the middle of the image there are two airplanes on the runway and there is a pole. There are two objects on the runway. \\
CAPTION: Two airplanes on an outdoors runway with buildings and sky on the background\\
\\
DESCRIPTION: Here in this picture we can see an air plane present in an airport over there and we can also see a couple of trucks present beside it over there and we can see people standing on the ground over there and in the far we can see trees and plants present over there.\\
CAPTION: An airplane in an airport with trucks beside it, there are people standing on the ground.\\
\\
DESCRIPTION: In this picture there is a view of the airport. In the front there is a white color tower and some flights parked on the ground. In the background there are some buildings. On the top we can see the plane flying in the sky.\\
CAPTION: An airport view, at the foreground a white color tower and planes parked on the ground. Building are present in the background and a plane is flying in the sky\\

DESCRIPTION: This picture is a black and white image. In this image we can see one woman with black sunglasses walking, some plants near the building, one big pole, some text on the bottom left side corner of the image, some grass on the ground, one object and one wire attached to the pole.\\
CAPTION: A black and white image of a woman walking with black sunglasses, a building is present also with plants near to it\\

DESCRIPTION: In this picture I can observe a man and woman. Woman is holding a paper in her hand. In the background I can observe a building and plants.\\
CAPTION: A man with a woman who is holding a paper in her hand, there is a building and plants at the background.\\
\\
DESCRIPTION: In this image I can see few women sitting on the concrete wall and I can see a dog which is brown, cream and black in color is sitting on the ground. In the background I can see a person standing, the white colored cloth, few plants and a table, and on the table I can see a white colored cloth.\\
CAPTION: Women sitting on the concrete wall outside a building with a brown, cream and black dog. At the background there is plants, a table and a person wearing white colored cloth\\
\\
DESCRIPTION: In this picture we can see a flower vase and a name board on the platform and here we can see four people are standing on the floor. In the background we can see the name on the wall and we can see plants, roof and lights.\\
CAPTION: \\

\midrule
Generated \\
\midrule
CAPTION: People standing on the floor near a flower vase and a name board.\\
\bottomrule
\end{tabular}   
\label{fig:prompt_ade20k_desc_to_caption}

\caption{Few-shot prompt example for generating a short and concise caption from a lengthy image description annotation for the Localized Narratives~\cite{pont2020connecting} datasets: ADE20k~\cite{ade20k_zhou2017scene} and OpenImages~\cite{openimages}.}

\end{figure*}


==> images/prompts/coco_relation.tex <==
\begin{figure*}
\centering
\footnotesize
\begin{tabular}{p{\linewidth}}
\toprule
Context \\
\midrule

Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.\\
\\
Guidelines:\\
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:\\
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., ``CAPTION: a blue ball on a shelf").\\
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., ``CONTRADICTION: green ball").\\
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\

\midrule
Few-Shot \\
\midrule

Guidelines:\\
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject\\
\\
Examples: \\
\\
CAPTION: ``A laptop next to a stack of books on a wooden desk"\\
CONTRADICTION: A laptop under a stack of books on a wooden desk.\\
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).\\
MISALIGNMENT TYPE: Relation\\
\\
CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .\\
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .\\
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)\\
MISALIGNMENT TYPE: Relation\\
\\
CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall\\
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall\\
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)\\
MISALIGNMENT TYPE: Relation\\
\\
CAPTION: Old fashioned chests are stacked atop each other on a city block.\\
CONTRADICTION: Old fashioned chests are stacked next to each other on a city block.\\
MISALIGNMENT: The chests are stacked atop each other (CAPTION: chests stacked atop each other), not next to each other (CONTRADICTION: chests stacked next to each other).\\
MISALIGNMENT TYPE: Relation\\
\\
CAPTION: Boy holding large stuffed toy bear outside of building.\\
CONTRADICTION: Boy holding large stuffed toy bear inside of building.\\
MISALIGNMENT: The boy is outside of a building (CAPTION: Boy holding large stuffed toy bear outside of building), not inside of it  (CONTRADICTION: boy holding large stuffed toy bear inside of building) .\\
MISALIGNMENT TYPE: Relation\\
\\
Create a MISALIGNMENT of type: Relation\\
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.\\
CAPTION: A crystal bowl filled with oranges on top of a table. \\

\midrule
Generated \\
\midrule
CONTRADICTION: A crystal bowl filled with oranges beneath a table.\\
MISALIGNMENT: The bowl is on top of the table (CAPTION: bowl on top of a table), not beneath it (CONTRADICTION: bowl beneath a table).\\
MISALIGNMENT TYPE: Relation\\

\bottomrule
\end{tabular}   
\caption{Few-shot prompt example for generating a \emph{Relation} misalignment in the COCO~\cite{COCO} dataset.}
\label{fig:prompt_coco_relation}

\end{figure*}


==> images/prompts/imagereward_noun.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \begin{tabular}{p{\linewidth}}
    \toprule
Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models. \\
\\
Guidelines:\\
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. \\
The elucidation should:\\
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").\\
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").\\
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\

\\
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.\\
\\
Examples: \\
\\
CAPTION: a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background\\
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background\\
MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure \\standing on a rock (CAPTION: robotic action figure standing on a rock)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background\\
CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background\\
MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .\\
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .\\
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a painting of a landscape with mountains and clouds in the sky\\
CONTRADICTION: a painting of a landscape with a beach and clouds in the sky\\
MISALIGNMENT: The painting is of a landscape with mountains (CAPTION: landscape with mountains) , not trees (CONTRADICTION: landscape with a beach) .\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: A black and green cat figurine on a gray surface.\\
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.\\
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a black and white drawing of a person wearing a helmet and headphones\\
CONTRADICTION: a black and white drawing of a person wearing a helmet and sunglasses\\
MISALIGNMENT: The person is wearing a headphone (CAPTION: person wearing a helmet and headphones), not sunglasses (CONTRADICTION: person wearing a helmet and sunglasses).\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a silhouette of a person standing in a forest with a castle in the background\\
CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background\\
MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand\\
CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water\\
MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)\\
MISALIGNMENT TYPE: Object/Noun\\
         \\
        \bottomrule
    \end{tabular}
    
    \caption{\color{red}WIP: Few-shot prompt example. This prompt is used to generate an \textit{object} misalignment type on ImageReward~\cite{xu2023imagereward} dataset.}
\end{figure*}


==> images/prompts/imagereward_noun2.tex <==
The following figures illustrate the formatting and phrasing of all the tasks included in the paper. All data comes from the ground truth datasets in this section, and no samples from GPT-3 are included here.


\begin{figure*} {  \footnotesize \begin{tabularx}{\linewidth}{r X} \toprule 
Context $\to$ &  Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models. \\
 \\
 & Guidelines:\\
 & Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
 & MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. \\
 & The elucidation should:\\
 & Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
 & For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").\\
 & For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").\\
 & MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\
\midrule
Few-Shot $\to$ &  Guidelines: \\
 & - Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.\\
\\
 & Examples: \\
\\
 & CAPTION: a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background\\
 & CONTRADICTION: a woman standing on a rock in the desert with mountains in the background\\
 & MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure standing on a rock (CAPTION: robotic action figure standing on a rock)\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background\\
 & CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background\\
 & MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .\\
 & CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .\\
 & MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: a painting of a landscape with mountains and clouds in the sky\\
 & CONTRADICTION: a painting of a landscape with a beach and clouds in the sky\\
 & MISALIGNMENT: The painting is of a landscape with mountains (CAPTION: landscape with mountains) , not trees (CONTRADICTION: landscape with a beach) .\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: A black and green cat figurine on a gray surface.\\
 & CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.\\
 & MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: a black and white drawing of a person wearing a helmet and headphones\\
 & CONTRADICTION: a black and white drawing of a person wearing a helmet and sunglasses\\
 & MISALIGNMENT: The person is wearing a headphone (CAPTION: person wearing a helmet and headphones), not sunglasses (CONTRADICTION: person wearing a helmet and sunglasses).\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: a silhouette of a person standing in a forest with a castle in the background\\
 & CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background\\
 & MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand\\
 & CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water\\
 & MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)\\
 & MISALIGNMENT TYPE: Object/Noun \\
 \\
 & CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand \\
\midrule
Generated $\to$ & CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand \\
 & CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water\\
 & MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)\\
 & MISALIGNMENT TYPE: Object/Noun \\
 \bottomrule 
 \end{tabularx} }  
 \caption{{\color{red} TODO!}}  
 \label{eval:RACE-h}  
 \end{figure*}

==> images/prompts/imagereward_noun3.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \begin{tabular}{p{\linewidth}}
    \toprule
Context\\
\midrule
Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models. \\
\\
Guidelines:\\
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. \\
The elucidation should:\\
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").\\
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").\\
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\
\midrule
Few-Shot \\
\midrule
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.\\
\\
Examples: \\
\\
CAPTION: a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background\\
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background\\
MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure \\standing on a rock (CAPTION: robotic action figure standing on a rock)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background\\
CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background\\
MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .\\
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .\\
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.\\
MISALIGNMENT TYPE: Object/Noun\\
 \\
CAPTION: a black and white drawing of a person wearing a helmet and headphones\\
CONTRADICTION: a black and white drawing of a person wearing a helmet and sunglasses\\
MISALIGNMENT: The person is wearing a headphone (CAPTION: person wearing a helmet and headphones), not sunglasses (CONTRADICTION: person wearing a helmet and sunglasses).\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a silhouette of a person standing in a forest with a castle in the background\\
CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background\\
MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand\\
CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water\\
MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
Create a MISALIGNMENT of type: Object/Noun \\
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it. \\
CAPTION: A samurai in armor and a helmet is holding a sword against a sunset sky with clouds\\

\midrule
Generation\\
\midrule
CAPTION: A samurai in armor and a helmet is holding a sword against a sunset sky with clouds\\
CONTRADICTION: A samurai in armor and a helmet is holding a gun against a sunset sky with clouds\\
MISALIGNMENT: The samurai is holding a sword (CAPTION: sword), not a gun (CONTRADICTION: gun)\\
MISALIGNMENT TYPE: Object/Noun\\
\bottomrule
\end{tabular}    
    \caption{\color{red}WIP: Few-shot prompt example. This prompt is used to generate an \textit{object} misalignment type on ImageReward~\cite{xu2023imagereward} dataset.}
\end{figure*}


==> images/prompts/pickapic_action.tex <==
\begin{figure*}
\centering
\footnotesize
\begin{tabular}{p{\linewidth}}
\toprule
Context \\
\midrule
Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.\\
Guidelines:\\
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. \\
The elucidation should:\\
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").\\
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").\\
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\
\midrule
Few-Shot \\
\midrule


Guidelines:\\
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.\\
\\
Examples: \\
\\
CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."\\
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.\\
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)\\
MISALIGNMENT TYPE: Action/Verb\\
\\
CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"\\
CONTRADICTION: a close up of a lion with a long mane drinking water on the grass in the forest with trees in the background\\
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion drinking water)\\
MISALIGNMENT TYPE: Action/Verb\\
\\
CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."\\
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .\\
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)\\
MISALIGNMENT TYPE: Action/Verb\\
\\
CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."\\
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.\\
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)\\
MISALIGNMENT TYPE: Action/Verb\\
\\
CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the background"\\
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background\\
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)\\
MISALIGNMENT TYPE: Action/Verb\\
\\
CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.\\
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.\\
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)\\
MISALIGNMENT TYPE: Action/Verb\\
\\
Create a MISALIGNMENT of type: Action/Verb\\
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.\\
CAPTION: A white cat is sitting on the grass in front of a house with trees and a blue sky in the background \\

\midrule
Generated \\
\midrule
CAPTION: A white cat is sitting on the grass in front of a house with trees and a blue sky in the background .\\
CONTRADICTION: A white cat is running on the grass in front of a house with trees and a blue sky in the background.\\
MISALIGNMENT: The cat is not running (CONTRADICTION: cat running), instead is sitting on the grass (CAPTION: cat sitting)\\
MISALIGNMENT TYPE: Action/Verb\\



\\
% CONGEN_SAMPLE = Create a MISALIGNMENT of type: misalignment_type
% Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.
% CAPTION: <context_captions>



\bottomrule
\end{tabular}   
\caption{Few-shot prompt example for generating an \emph{Action} misalignment in the PickaPic~\cite{Kirstain2023PickaPicAO} dataset.}
\label{fig:prompt_pickapic_action}

\end{figure*}


==> images/prompts/raw_prompts/coco.tex <==
OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A stained glass window with a cartoon image of a man with glasses and a beard .
CONTRADICTION: A stained glass window with a cartoon image of a man with a beard .
MISALIGNMENT: The man in stained glass wear glasses (CAPTION: man with glasses and a beard), instead of only beard (CONTRADICTION: man with a beard).
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A sign welcomes visitors to Lake Kawaguchiko in English and in another language.
CONTRADICTION: A mascot welcomes visitors to Lake Kawaguchiko in Japanese and in another language.
MISALIGNMENT: There is a sign welcoming visitors to Lake Kawaguchiko (CAPTION: sign), not a mascot (CONTRADICTION: mascot)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Two dogs on a leash playing on the shore and in the water of a lake.
CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano.
MISALIGNMENT: The dogs are playing on the shore and in the water of a lake (CAPTION: Two dogs on a leash playing on the shore and in the water of a lake), not a volcano (CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano).
MISALIGNMENT TYPE: Object/Noun

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Three pigeons on the side walk munching on a thrown out breadstick.
CONTRADICTION: Eight pigeons on the side walk munching on a thrown out pizza crust.
MISALIGNMENT: There are three pigeons eating a breadstick (CAPTION: Three pigeons munching on a breadstick), not eight. (CONTRADICTION: Eight pigeons munching on a breadstick)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A box of pizza with peppers, onions and sausage on it.
CONTRADICTION: A box of pizza with pineapple on it.
MISALIGNMENT: The pizza has peppers, onions and mushrooms on it (CAPTION: peppers, onions and mushrooms), not pineapple (CONTRADICTION: pineapple)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A baseball player holding a bat while standing next to a home plate.
CONTRADICTION: A baseball player holding a bat while standing next to Batman.
MISALIGNMENT: The baseball player is not holding a bat next to Batman (CONTRADICTION: player next to Batman) , instead is next to a home plate (CAPTION: player next to home plate) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A woman playing tennis is swinging at a tennis ball.
CONTRADICTION: A woman playing tennis is juggling tennis balls.
MISALIGNMENT: The woman is swinging at a tennis ball (CAPTION: woman playing tennis is swinging at a tennis ball), not juggling tennis balls (CONTRADICTION: woman playing tennis is juggling tennis balls).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A bird is sitting on a branch eating a banana peel.
CONTRADICTION: A bird is sitting on a branch eating an apple.
MISALIGNMENT: The bird is eating an apple (CAPTION: bird eating an apple), not a banana peel (CONTRADICTION: bird eating a banana peel).
MISALIGNMENT TYPE: Object/Noun
"""

ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"
CONTRADICTION: a cartoon of a mermaid with black hair in the water
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with black hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A cartoon drawing of a person with bat wings on a white paper with a keyboard and pens on a table ."
CONTRADICTION: A cartoon drawing of a person with angel wings on a white paper with a keyboard and pens on a table.
MISALIGNMENT: The person wings are bat wings (CAPTION: person with bat wings), not angel wings (CONTRADICTION: person with angle wings).
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a naked woman with long hair on a grey background
CONTRADICTION: A portrait of a naked woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: The colorful flowers are in the vase next to the window.
CONTRADICTION: The white and black flowers are in the vase next to the window.
MISALIGNMENT: The flowers are colorful (CAPTION: colorful flowers) , not white and black (CONTRADICTION: white and black flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: Vase sitting next to the window with droopy flowers in it.
CONTRADICTION: Vase sitting next to the window with fresh flowers in it.
MISALIGNMENT: The vase has droppy flowers (CAPTION: droppy flowers), not fresh flowers (CAPTION: fresh flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A bicycle chained to a red pole and a green pole on the sidewalk in front of a building.
CONTRADICTION: A bicycle chained to a red pole and a blue pole on the sidewalk in front of a building.
MISALIGNMENT: One of the poles is red (CAPTION: green pole), not blue (CONTRADICTION: blue pole)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a kid trying to use a skating board on the road
CONTRADICTION: a kid breaking a skating board on the road
MISALIGNMENT: The kid is trying to use a skating board (CAPTION: kid trying to use a skating board), not breaking it (CONTRADICTION: kid breaking a skating board)
MISALIGNMENT TYPE: Action/Verb

CAPTION: Seated person wearing blue jeans holding a white corded electronic device.
CONTRADICTION: Seated person wearing blue jeans chewing a white cordless electronic device.
MISALIGNMENT: The person is holding a corded electronic device (CAPTION: person holding a white corded electronic device), not chewing a corded electronic device (CONTRADICTION: person chewing a corded electronic device)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A cup, saucer and spoon sitting next to a newspaper.
CONTRADICTION: A cup, saucer, and spoon flying next to a newspaper.
MISALIGNMENT: The cup, saucer, and spoon are sitting (CAPTION: cup, saucer, and spoon sitting next to a newspaper), not flying (CONTRADICTION: cup, saucer, and spoon flying next to a newspaper).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A man that is standing in the grass with a kite.
Contradiction: A man that is lying in the grass with a kite.
Misalignment: The man is standing (CAPTION: man standing in the grass with a kite), not lying (CONTRADICTION: man lying in the grass with a kite).
Misalignment Type: Action/Verb

"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation

CAPTION: Old fashioned chests are stacked atop each other on a city block.
CONTRADICTION: Old fashioned chests are stacked next to each other on a city block.
MISALIGNMENT: The chests are stacked atop each other (CAPTION: chests stacked atop each other), not next to each other (CONTRADICTION: chests stacked next to each other).
MISALIGNMENT TYPE: Relation

CAPTION: Boy holding large stuffed toy bear outside of building.
CONTRADICTION: Boy holding large stuffed toy bear inside of building.
MISALIGNMENT: The boy is outside of a building (CAPTION: Boy holding large stuffed toy bear outside of building), not inside of it  (CONTRADICTION: boy holding large stuffed toy bear inside of building) .
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation
"""

CONGEN_SAMPLE = """Create a MISALIGNMENT of type: <misalignment_type>
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.
CAPTION: <context_captions>
"""


==> images/prompts/raw_prompts/flickr30k.tex <==
BASE_CONGEN_PROMPT_V3_MERGED_MISALIGNMENT = """Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.

Guidelines:
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation
"""

OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A stained glass window with a cartoon image of a man with glasses and a beard .
CONTRADICTION: A stained glass window with a cartoon image of a man with a beard .
MISALIGNMENT: The man in stained glass wear glasses (CAPTION: man with glasses and a beard), instead of only beard (CONTRADICTION: man with a beard).
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A sign welcomes visitors to Lake Kawaguchiko in English and in another language.
CONTRADICTION: A mascot welcomes visitors to Lake Kawaguchiko in Japanese and in another language.
MISALIGNMENT: There is a sign welcoming visitors to Lake Kawaguchiko (CAPTION: sign), not a mascot (CONTRADICTION: mascot)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Two dogs on a leash playing on the shore and in the water of a lake.
CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano.
MISALIGNMENT: The dogs are playing on the shore and in the water of a lake (CAPTION: Two dogs on a leash playing on the shore and in the water of a lake), not a volcano (CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano).
MISALIGNMENT TYPE: Object/Noun

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Three pigeons on the side walk munching on a thrown out breadstick.
CONTRADICTION: Eight pigeons on the side walk munching on a thrown out pizza crust.
MISALIGNMENT: There are three pigeons eating a breadstick (CAPTION: Three pigeons munching on a breadstick), not eight. (CONTRADICTION: Eight pigeons munching on a breadstick)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A box of pizza with peppers, onions and sausage on it.
CONTRADICTION: A box of pizza with pineapple on it.
MISALIGNMENT: The pizza has peppers, onions and mushrooms on it (CAPTION: peppers, onions and mushrooms), not pineapple (CONTRADICTION: pineapple)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A baseball player holding a bat while standing next to a home plate.
CONTRADICTION: A baseball player holding a bat while standing next to Batman.
MISALIGNMENT: The baseball player is not holding a bat next to Batman (CONTRADICTION: player next to Batman) , instead is next to a home plate (CAPTION: player next to home plate) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A woman playing tennis is swinging at a tennis ball.
CONTRADICTION: A woman playing tennis is juggling tennis balls.
MISALIGNMENT: The woman is swinging at a tennis ball (CAPTION: woman playing tennis is swinging at a tennis ball), not juggling tennis balls (CONTRADICTION: woman playing tennis is juggling tennis balls).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A bird is sitting on a branch eating a banana peel.
CONTRADICTION: A bird is sitting on a branch eating an apple.
MISALIGNMENT: The bird is eating an apple (CAPTION: bird eating an apple), not a banana peel (CONTRADICTION: bird eating a banana peel).
MISALIGNMENT TYPE: Object/Noun
"""


ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"
CONTRADICTION: a cartoon of a mermaid with black hair in the water
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with black hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A cartoon drawing of a person with bat wings on a white paper with a keyboard and pens on a table ."
CONTRADICTION: A cartoon drawing of a person with angel wings on a white paper with a keyboard and pens on a table.
MISALIGNMENT: The person wings are bat wings (CAPTION: person with bat wings), not angel wings (CONTRADICTION: person with angle wings).
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a naked woman with long hair on a grey background
CONTRADICTION: A portrait of a naked woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: The colorful flowers are in the vase next to the window.
CONTRADICTION: The white and black flowers are in the vase next to the window.
MISALIGNMENT: The flowers are colorful (CAPTION: colorful flowers) , not white and black (CONTRADICTION: white and black flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: Vase sitting next to the window with droopy flowers in it.
CONTRADICTION: Vase sitting next to the window with fresh flowers in it.
MISALIGNMENT: The vase has droppy flowers (CAPTION: droppy flowers), not fresh flowers (CAPTION: fresh flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A bicycle chained to a red pole and a green pole on the sidewalk in front of a building.
CONTRADICTION: A bicycle chained to a red pole and a blue pole on the sidewalk in front of a building.
MISALIGNMENT: One of the poles is red (CAPTION: green pole), not blue (CONTRADICTION: blue pole)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a kid trying to use a skating board on the road
CONTRADICTION: a kid breaking a skating board on the road
MISALIGNMENT: The kid is trying to use a skating board (CAPTION: kid trying to use a skating board), not breaking it (CONTRADICTION: kid breaking a skating board)
MISALIGNMENT TYPE: Action/Verb

CAPTION: Seated person wearing blue jeans holding a white corded electronic device.
CONTRADICTION: Seated person wearing blue jeans chewing a white cordless electronic device.
MISALIGNMENT: The person is holding a corded electronic device (CAPTION: person holding a white corded electronic device), not chewing a corded electronic device (CONTRADICTION: person chewing a corded electronic device)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A cup, saucer and spoon sitting next to a newspaper.
CONTRADICTION: A cup, saucer, and spoon flying next to a newspaper.
MISALIGNMENT: The cup, saucer, and spoon are sitting (CAPTION: cup, saucer, and spoon sitting next to a newspaper), not flying (CONTRADICTION: cup, saucer, and spoon flying next to a newspaper).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A man that is standing in the grass with a kite.
CONTRADICTION: A man that is lying in the grass with a kite.
MISALIGNMENT: The man is standing (CAPTION: man standing in the grass with a kite), not lying (CONTRADICTION: man lying in the grass with a kite).
MISALIGNMENT TYPE: Action/Verb

CAPTION: a man sleeping on a bench outside with a white and black dog sitting next to him .
CONTRADICTION: a man sleeping on a bench outside with a white and black dog running next to him .
MISALIGNMENT: The dog is running (CAPTION: dog running), not sitting (CONTRADICTION: dog sitting)
MISALIGNMENT TYPE: Action/Verb
"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation

CAPTION: Old fashioned chests are stacked atop each other on a city block.
CONTRADICTION: Old fashioned chests are stacked next to each other on a city block.
MISALIGNMENT: The chests are stacked atop each other (CAPTION: chests stacked atop each other), not next to each other (CONTRADICTION: chests stacked next to each other).
MISALIGNMENT TYPE: Relation

CAPTION: Boy holding large stuffed toy bear outside of building.
CONTRADICTION: Boy holding large stuffed toy bear inside of building.
MISALIGNMENT: The boy is outside of a building (CAPTION: Boy holding large stuffed toy bear outside of building), not inside of it  (CONTRADICTION: boy holding large stuffed toy bear inside of building) .
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation
"""


==> images/prompts/raw_prompts/imagereward.tex <==
BASE_CONGEN_PROMPT_V3_MERGED_MISALIGNMENT = """Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.

Guidelines:
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation
"""

OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure standing on a rock (CAPTION: robotic action figure standing on a rock)
MISALIGNMENT TYPE: Object/Noun

CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background
CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background
MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: a painting of a landscape with mountains and clouds in the sky
CONTRADICTION: a painting of a landscape with a beach and clouds in the sky
MISALIGNMENT: The painting is of a landscape with mountains (CAPTION: landscape with mountains) , not trees (CONTRADICTION: landscape with a beach) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: a black and white drawing of a person wearing a helmet and headphones
CONTRADICTION: a black and white drawing of a person wearing a helmet and sunglasses
MISALIGNMENT: The person is wearing a headphone (CAPTION: person wearing a helmet and headphones), not sunglasses (CONTRADICTION: person wearing a helmet and sunglasses).
MISALIGNMENT TYPE: Object/Noun

CAPTION: a silhouette of a person standing in a forest with a castle in the background
CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background
MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)
MISALIGNMENT TYPE: Object/Noun

CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand
CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water
MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)
MISALIGNMENT TYPE: Object/Noun
"""

ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: a gold coin with a logo on it on a gray wall
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a waterfall in a tropical forest with green plants and trees
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A cartoon drawing of a person with bat wings on a white paper with a keyboard and pens on a table .
CONTRADICTION: A cartoon drawing of a person with angel wings on a white paper with a keyboard and pens on a table.
MISALIGNMENT: The person wings are bat wings (CAPTION: person with bat wings), not angel wings (CONTRADICTION: person with angle wings).
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a woman with long hair on a grey background
CONTRADICTION: A portrait of a woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A futuristic spider toy and a robotic spider toy on a gray surface .
CONTRADICTION: A futuristic spider toy and a plastic spider toy on a gray surface
MISALIGNMENT: The spider toy is robotic (CONTRADICTION: robotic spider toy), not plastic (CAPTION: plastic spider toy)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a black and white drawing of a light fixture with a gray background
CONTRADICTION: A colorful drawing of a light fixture with a gray background
MISALIGNMENT: The drawing is not colorful (CONTRADICTION: colorful drawing) , instead is black and white (CAPTION: black and white drawing) .
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a painting of a skeleton person with a skull face and a hooded person with a skull face
CONTRADICTION: A painting of a real person with a skull face and a hooded person with a skull face
MISALIGNMENT: The person is not real (CONTRADICTION: real person), but a skeleton (CAPTION: skeleton person)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A black and white portrait of a bald man with glasses and a beard .
CONTRADICTION: A black and white portrait of a bald man with glasses and an eyepatch
MISALIGNMENT: The man has glasses and beard (CONTRADICTION: man with glasses and a beard), not glasses and eyepatch (CAPTION: man with glasses and an eyepatch) .
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a red color smoke coming from a fire in the sky with clouds and grass on the ground
CONTRADICTION: a blue color smoke coming from a fire in the sky with clouds and grass on the ground
MISALIGNMENT: The smoke is red (CAPTION: red color smoke), not blue (CONTRADICTION: blue color smoke)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane drinking water on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion drinking water)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A cartoon of a man in a suit and hat sitting at a table in a city with buildings and a blue sky."
CONTRADICTION: A cartoon of a man in a suit and hat jumping on a table in a city with buildings and a blue sky.
MISALIGNMENT: The man is not jumping (CONTRADICTION: man in a suit and hat jumping) , instead is sitting at the table (CAPTION: man in a suit and hat sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a futuristic spaceship flying in the sky with clouds and stars in the background
CONTRADICTION: a futuristic spaceship explodes in the sky with clouds and stars in the background
MISALIGNMENT: The spaceship is not exploded (CONTRADICTION: spaceship explodes), instead is flying (CAPTION: spaceship flying)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a fantasy painting of a forest with a river flowing through it and trees in the background
"CONTRADICTION: a fantasy painting of a forest with a river freeze through it and trees in the background
MISALIGNMENT: The river is flowing (CONTRADICTION: river flowing), not freeze (CAPTION: river freeze)
MISALIGNMENT TYPE: Action/Verb"
"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: a black and white drawing of a light fixture with a gray background
CONTRADICTION: A colorful drawing of a light fixture with a gray background
MISALIGNMENT: The drawing is not colorful (CONTRADICTION: colorful drawing) , instead is black and white (CAPTION: black and white drawing) .
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a futuristic spaceship flying in the sky with clouds and stars in the background
CONTRADICTION: a futuristic spaceship explodes in the sky with clouds and stars in the background
MISALIGNMENT: The spaceship is not exploded (CONTRADICTION: spaceship explodes), instead is flying (CAPTION: spaceship flying)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a silhouette of a person standing in a forest with a castle in the background
CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background
MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)
MISALIGNMENT TYPE: Object/Noun
"""


==> images/prompts/raw_prompts/localized_narratives.tex <==
BASE_CONGEN_PROMPT_V3_MERGED_MISALIGNMENT = """Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.

Guidelines:
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation
"""

OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A sign welcomes visitors to Lake Kawaguchiko in English and in another language.
CONTRADICTION: A mascot welcomes visitors to Lake Kawaguchiko in Japanese and in another language.
MISALIGNMENT: There is a sign welcoming visitors to Lake Kawaguchiko (CAPTION: sign), not a mascot (CONTRADICTION: mascot)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Two dogs on a leash playing on the shore and in the water of a lake.
CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano.
MISALIGNMENT: The dogs are playing on the shore and in the water of a lake (CAPTION: Two dogs on a leash playing on the shore and in the water of a lake), not a volcano (CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano).
MISALIGNMENT TYPE: Object/Noun

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Three pigeons on the side walk munching on a thrown out breadstick.
CONTRADICTION: Eight pigeons on the side walk munching on a thrown out pizza crust.
MISALIGNMENT: There are three pigeons eating a breadstick (CAPTION: Three pigeons munching on a breadstick), not eight. (CONTRADICTION: Eight pigeons munching on a breadstick)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A box of pizza with peppers, onions and sausage on it.
CONTRADICTION: A box of pizza with pineapple on it.
MISALIGNMENT: The pizza has peppers, onions and mushrooms on it (CAPTION: peppers, onions and mushrooms), not pineapple (CONTRADICTION: pineapple)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A baseball player holding a bat while standing next to a home plate.
CONTRADICTION: A baseball player holding a bat while standing next to Batman.
MISALIGNMENT: The baseball player is not holding a bat next to Batman (CONTRADICTION: player next to Batman) , instead is next to a home plate (CAPTION: player next to home plate) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A woman playing tennis is swinging at a tennis ball.
CONTRADICTION: A woman playing tennis is juggling tennis balls.
MISALIGNMENT: The woman is swinging at a tennis ball (CAPTION: woman playing tennis is swinging at a tennis ball), not juggling tennis balls (CONTRADICTION: woman playing tennis is juggling tennis balls).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A bird is sitting on a branch eating a banana peel.
CONTRADICTION: A bird is sitting on a branch eating an apple.
MISALIGNMENT: The bird is eating an apple (CAPTION: bird eating an apple), not a banana peel (CONTRADICTION: bird eating a banana peel).
MISALIGNMENT TYPE: Object/Noun

CAPTION: A room with a chandelier, chairs and pillars.
CONTRADICTION: A room with a fountain, chairs and a table.
MISALIGNMENT: The room has a chandelier (CAPTION: a chandelier) , instead of a fountain (CONTRADICTION: a fountain) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A view of a mountain range with grass, plants, and trees.
CONTRADICTION: A view of a mountain range with grass, plants, and a lake.
MISALIGNMENT: There are grass, plants and trees in the view (CAPTION: mountain range with grass, plants, and trees) , no lake (CONTRADICTION: mountain range with grass, plants, and a lake.)
MISALIGNMENT TYPE: Object/Noun
"""


ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"
CONTRADICTION: a cartoon of a mermaid with black hair in the water
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with black hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a naked woman with long hair on a grey background
CONTRADICTION: A portrait of a naked woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: The colorful flowers are in the vase next to the window.
CONTRADICTION: The white and black flowers are in the vase next to the window.
MISALIGNMENT: The flowers are colorful (CAPTION: colorful flowers) , not white and black (CONTRADICTION: white and black flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: Vase sitting next to the window with droopy flowers in it.
CONTRADICTION: Vase sitting next to the window with fresh flowers in it.
MISALIGNMENT: The vase has droppy flowers (CAPTION: droppy flowers), not fresh flowers (CAPTION: fresh flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A bicycle chained to a red pole and a green pole on the sidewalk in front of a building.
CONTRADICTION: A bicycle chained to a red pole and a blue pole on the sidewalk in front of a building.
MISALIGNMENT: One of the poles is red (CAPTION: green pole), not blue (CONTRADICTION: blue pole)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a kid trying to use a skating board on the road
CONTRADICTION: a kid breaking a skating board on the road
MISALIGNMENT: The kid is trying to use a skating board (CAPTION: kid trying to use a skating board), not breaking it (CONTRADICTION: kid breaking a skating board)
MISALIGNMENT TYPE: Action/Verb

CAPTION: Seated person wearing blue jeans holding a white corded electronic device.
CONTRADICTION: Seated person wearing blue jeans chewing a white cordless electronic device.
MISALIGNMENT: The person is holding a corded electronic device (CAPTION: person holding a white corded electronic device), not chewing a corded electronic device (CONTRADICTION: person chewing a corded electronic device)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A cup, saucer and spoon sitting next to a newspaper.
CONTRADICTION: A cup, saucer, and spoon flying next to a newspaper.
MISALIGNMENT: The cup, saucer, and spoon are sitting (CAPTION: cup, saucer, and spoon sitting next to a newspaper), not flying (CONTRADICTION: cup, saucer, and spoon flying next to a newspaper).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A man that is standing in the grass with a kite.
Contradiction: A man that is lying in the grass with a kite.
Misalignment: The man is standing (CAPTION: man standing in the grass with a kite), not lying (CONTRADICTION: man lying in the grass with a kite).
Misalignment Type: Action/Verb

CAPTION: A woman stands while people sit at a table.
CONTRADICTION: A woman sits while people stand at a table.
MISALIGNMENT: The woman is standing (CAPTION: woman stands), not sitting (CONTRADICTION: woman sits)
MISALIGNMENT TYPE: Action/Verb
"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation

CAPTION: Old fashioned chests are stacked atop each other on a city block.
CONTRADICTION: Old fashioned chests are stacked next to each other on a city block.
MISALIGNMENT: The chests are stacked atop each other (CAPTION: chests stacked atop each other), not next to each other (CONTRADICTION: chests stacked next to each other).
MISALIGNMENT TYPE: Relation

CAPTION: Boy holding large stuffed toy bear outside of building.
CONTRADICTION: Boy holding large stuffed toy bear inside of building.
MISALIGNMENT: The boy is outside of a building (CAPTION: Boy holding large stuffed toy bear outside of building), not inside of it  (CONTRADICTION: boy holding large stuffed toy bear inside of building) .
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation
"""


CONGEN_SAMPLE = """Create a MISALIGNMENT of type: <misalignment_type>
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.
CAPTION: <context_captions>
"""

==> images/prompts/raw_prompts/pickapic.tex <==
BASE_CONGEN_PROMPT_V3_MERGED_MISALIGNMENT = """Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.

Guidelines:
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation
"""

OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure standing on a rock (CAPTION: robotic action figure standing on a rock)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a painting of a ballroom with a chandelier hanging from the ceiling and two persons standing on the floor"
CONTRADICTION: a painting of a bedroom with a chandelier hanging from the ceiling and two persons standing on the floor
MISALIGNMENT: The scene is of a ballroom (CAPTION: ballroom with a chandelier), not a bedroom (CONTRADICTION: bedroom)
MISALIGNMENT TYPE: Object/Noun

CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background
CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background
MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A stained glass window with a cartoon image of a man with glasses and a beard .
CONTRADICTION: A stained glass window with a cartoon image of a man with a beard .
MISALIGNMENT: The man in stained glass wear glasses (CAPTION: man with glasses and a beard), instead of only beard (CONTRADICTION: man with a beard).
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun
"""

ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"
CONTRADICTION: a cartoon of a mermaid with long black hair in the water
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with long black hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A cartoon drawing of a person with bat wings on a white paper with a keyboard and pens on a table ."
CONTRADICTION: A cartoon drawing of a person with angel wings on a white paper with a keyboard and pens on a table.
MISALIGNMENT: The person wings are bat wings (CAPTION: person with bat wings), not angel wings (CONTRADICTION: person with angle wings).
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a woman with long hair on a grey background
CONTRADICTION: A portrait of a woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane drinking water on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion drinking water)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A cartoon of a man in a suit and hat sitting at a table in a city with buildings and a blue sky."
CONTRADICTION: A cartoon of a man in a suit and hat jumping on a table in a city with buildings and a blue sky.
MISALIGNMENT: The man is not jumping (CONTRADICTION: man in a suit and hat jumping) , instead is sitting at the table (CAPTION: man in a suit and hat sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb
"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation
"""

CONGEN_SAMPLE = """Create a MISALIGNMENT of type: <misalignment_type>
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.
CAPTION: <context_captions>
"""


==> images/prompts/raw_prompts/seetrue.tex <==
BASE_CONGEN_PROMPT = """Your primary task is to generate a single summarized feedback based on visual feedback provided in the input, and identify the source of misalignment between the caption and the visual content. The goal is to extract meaningful insights from the feedback and link them to the corresponding elements in the caption.

Guidelines:
SUMMARIZED FEEDBACK: Given a caption and a set of visual feedbacks, your objective is to create a concise and informative feedback statement that captures the most significant misalignment between the caption and the visual content. No need to mention "at the caption" or "at the image".
Misalignment Identification: After constructing the summarized feedback, you should indicate the source of misalignment for both the caption and the visual content. In parentheses, specify the origin of the misalignment as follows:
CAPTION: Describe the source of misalignment that originates from the text (e.g., a description or detail in the caption that does not match the image). Mention also the related subject.
CONTRADICTION: Based on the feedback, pinpoint the source of misalignment in the visual content that contradicts the caption. Make sure the CONTRADICTION referes only to the relative part in FEEDBACKS. Mention also the related subject.


Examples:

CAPTION: "A woman with a blue shirt and yellow flower headband, sitting on a wooden bench outside on the grass."
FEEDBACKS: ["The woman's shirt is yellow, not blue.", "The woman sitting on the wooden bench is wearing a white shirt, not a blue shirt.", "The woman has a yellow shirt on, not blue."]
MISALIGNMENT: The sitting woman is wearing a yellow shirt (CONTRADICTION: yellow shirt), not a blue shirt (CAPTION: blue shirt)

CAPTION: "A banana on the left of an apple."
FEEDBACKS: ["The banana is to the right of the apple, not to its left.", "A banana on the right of an apple, not the left.", "The apple is to the left of a yellow pepper, but there is not a banana to the left of the apple"]
MISALIGNMENT: The banana is not on the left of the apple (CAPTION: banana left of an apple), instead it's on the right (CONTRADICTION: banana right of the apple)

CAPTION: "A donkey and an octopus are playing a game. The donkey is holding a rope on one end, the octopus is holding onto the other. The donkey holds the rope in its mouth. A cat is jumping over the rope."
FEEDBACKS: ["An octopus jumped over the rope, not a cat.", NaN, "There are three creatures, but no octopus or donkey"]
MISALIGNMENT: There are three creatures (CONTRADICTION: three creatures), but no donkey, octopus and cat (CAPTION: A donkey and an octopus. cat jumping rope).

CAPTION: A couch on the left of a chair.
FEEDBACKS: ["A couch is to the left of a coffee table, there is no chair present.", "A couch and two tables under a window, there is no chair.", NaN]
MISALIGNMENT: The couch is to the left of a table (CONTRADICTION: coffe table), not left of a chair (CAPTION: chair).

CAPTION: A sheep to the right of a wine glass.
FEEDBACKS: ["A sheep is facing the camera, not to the right of a wine glass, which is not present.", "A sheep looking at the camera, there is no wine glass.", "There is only a sheep alone in a field, it is not to the right of a wine glass"]
MISALIGNMENT: There is no wine glass (CAPTION: wine glass) (CONTRADICTION: no wine glass)

CAPTION: A tomato has been put on top of a pumpkin on a kitchen stool. There is a fork sticking into the pumpkin. The scene is viewed from above.
FEEDBACKS: [NaN, "A pumpkin has been put on top of a kitchen stool. There is a fork sticking into the pumpkin. The scene is viewed from above. There is no tomato on top of the pumpkin.", "There is only a pumpkin, and no tomato"]
MISALIGNMENT: There is no tomato on top of a pumpkin (CAPTION: tomato on top of a pumpkin) (CONTRADICTION: no tomato)

CAPTION: a red glass ball with a reflection on top of a gray surface
FEEDBACKS: ["The glass ball is blue, not red.", "The ball with the reflection should be blue instead of red.", "The ball is blue, not red"]
MISALIGNMENT: The color of the ball is blue (CONTRADICTION: blue ball), not red (CAPTION: red ball)

CAPTION: A lunch salad in a yellow bowl made out of fruit, vegetables, and meats with chopsticks. 
FEEDBACKS: ["There is no meat present, nor are there any chopsticks, simply the bowl with fruit and vegetable.", "There is a bowl of food, but no chopsticks.", "There is a salad with fruit and vegetables in a yellow bowl but there does not appear to be meat in it and there are no chopsticks."]
MISALIGNMENT: There is a yellow bowl with fruit and vegetables (CONTRADICTION: salad with fruit and vegetables in a yellow bowl) but without meat, also no chopsticks present (CAPTION: salad made out of fruit, vegetables, and meats with chopsticks)

CAPTION: A cup filled with umbrellas and canes next to a white wall.
FEEDBACKS: ["The wall is gray, not white.", "A bucket has two canes in it, not umbrellas and canes and it is front of a gray wall, not a white wall.", "A cup has canes in it, but no umbrellas"]
MISALIGNMENT: The cup has canes in it (CAPTION: umbrellas and canes), but no umbrellas (CONTRADICTION: no umbrellas). The wall is not white (CAPTION: white tall), instead is gray (CONTRADICTION: gray wall).

CAPTION: Small white toilet with spare rolls of toilet paper beside it.
FEEDBACKS:["A small white toilet is here without any rolls of toilet paper, not any spares.", "There is a toilet but no toilet paper.", "The toilet only has curtains/walls next to it, not spare rolls of toilet paper."]
MISALIGNMENT: The toilet does not have any spare rolls of toilet paper beside it (CONTRADICTION: NO toilet paper), as described in the caption (CAPTION: spare rolls of toilet paper)

CAPTION: the woman wearing red is looking at a pool in front of a brown building
FEEDBACKS:["A woman wearing red is standing with her back to a pool, not looking at it.", "The building is white not brown.", NaN]
MISALIGNMENT: The woman is standing with her back to a pool (CONTRADICTION: woman standing with her back to a pool), as described in the caption (CAPTION: woman looking at a pool). The building is white (CONTRADICTION: white building), not brown (CAPTION: brown building)

CAPTION: A yellow and green fire hydrant in Canada.
FEEDBACKS:["There is an all green fire hydrant, whose location could be anywhere, but isn't specifically Canadian.", "The hydrant is only green, not yellow and green.", "The fire hydrant is green and black, not green and yellow."]
MISALIGNMENT: The fire hydrant is only green (CONTRADICTION: green fire hydrant), not yellow and green (CAPTION: yellow and green fire hydrant).
"""

SAMPLETEMPLATE = """CAPTION: <caption>
FEEDBACKS: <feedback>
MISALIGNMENT:
"""


==> images/prompts/seetrue_prompt.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \begin{tabular}{p{\linewidth}}
    \toprule
Context\\
\midrule
Your primary task is to generate a single summarized feedback based on visual feedback provided in the input, and identify the source of misalignment between the caption and the visual content. The goal is to extract meaningful insights from the feedback and link them to the corresponding elements in the caption.\\

Guidelines:\\
SUMMARIZED FEEDBACK: Given a caption and a set of visual feedbacks, your objective is to create a concise and informative feedback statement that captures the most significant misalignment between the caption and the visual content. No need to mention "at the caption" or "at the image".\\
Misalignment Identification: After constructing the summarized feedback, you should indicate the source of misalignment for both the caption and the visual content. In parentheses, specify the origin of the misalignment as follows:\\
CAPTION: Describe the source of misalignment that originates from the text (e.g., a description or detail in the caption that does not match the image). Mention also the related subject.\\
CONTRADICTION: Based on the feedback, pinpoint the source of misalignment in the visual content that contradicts the caption. Make sure the CONTRADICTION refers only to the relative part in FEEDBACKS. Mention also the related subject.\\
\midrule
Few-Shot \\
\midrule
Examples:\\
\\
CAPTION: "A woman with a blue shirt and yellow flower headband, sitting on a wooden bench outside on the grass."\\
FEEDBACKS: ["The woman's shirt is yellow, not blue.", "The woman sitting on the wooden bench is wearing a white shirt, not a blue shirt.", "The woman has a yellow shirt on, not blue."]\\
MISALIGNMENT: The sitting woman is wearing a yellow shirt (CONTRADICTION: yellow shirt), not a blue shirt (CAPTION: blue shirt)\\
\\
CAPTION: A couch on the left of a chair.\\
FEEDBACKS: ["A couch is to the left of a coffee table, there is no chair present.", "A couch and two tables under a window, there is no chair.", NaN]\\
MISALIGNMENT: The couch is to the left of a table (CONTRADICTION: coffe table), not left of a chair (CAPTION: chair).\\
\\
CAPTION: A sheep to the right of a wine glass.\\
FEEDBACKS: ["A sheep is facing the camera, not to the right of a wine glass, which is not present.", "A sheep looking at the camera, there is no wine glass.", "There is only a sheep alone in a field, it is not to the right of a wine glass"]\\
MISALIGNMENT: There is no wine glass (CAPTION: wine glass) (CONTRADICTION: no wine glass)\\
\\
CAPTION: A tomato has been put on top of a pumpkin on a kitchen stool. There is a fork sticking into the pumpkin. The scene is viewed from above.\\
FEEDBACKS: [NaN, "A pumpkin has been put on top of a kitchen stool. There is a fork sticking into the pumpkin. The scene is viewed from above. There is no tomato on top of the pumpkin.", "There is only a pumpkin, and no tomato"]\\
MISALIGNMENT: There is no tomato on top of a pumpkin (CAPTION: tomato on top of a pumpkin) (CONTRADICTION: no tomato)\\
\\
CAPTION: a red glass ball with a reflection on top of a gray surface\\
FEEDBACKS: ["The glass ball is blue, not red.", "The ball with the reflection should be blue instead of red.", "The ball is blue, not red"]\\
MISALIGNMENT: The color of the ball is blue (CONTRADICTION: blue ball), not red (CAPTION: red ball)\\
\\
CAPTION: A lunch salad in a yellow bowl made out of fruit, vegetables, and meats with chopsticks. \\
FEEDBACKS: ["There is no meat present, nor are there any chopsticks, simply the bowl with fruit and vegetable.", "There is a bowl of food, but no chopsticks.", "There is a salad with fruit and vegetables in a yellow bowl but there does not appear to be meat in it and there are no chopsticks."]\\
MISALIGNMENT: There is a yellow bowl with fruit and vegetables (CONTRADICTION: salad with fruit and vegetables in a yellow bowl) but without meat, also no chopsticks present (CAPTION: salad made out of fruit, vegetables, and meats with chopsticks)\\
\\
CAPTION: A cup filled with umbrellas and canes next to a white wall.\\
FEEDBACKS: ["The wall is gray, not white.", "A bucket has two canes in it, not umbrellas and canes and it is front of a gray wall, not a white wall.", "A cup has canes in it, but no umbrellas"]\\
MISALIGNMENT: The cup has canes in it (CAPTION: umbrellas and canes), but no umbrellas (CONTRADICTION: no umbrellas). The wall is not white (CAPTION: white tall), instead is gray (CONTRADICTION: gray wall).\\
\\
CAPTION: Small white toilet with spare rolls of toilet paper beside it.\\
FEEDBACKS:["A small white toilet is here without any rolls of toilet paper, not any spares.", "There is a toilet but no toilet paper.", "The toilet only has curtains/walls next to it, not spare rolls of toilet paper."]\\
MISALIGNMENT: The toilet does not have any spare rolls of toilet paper beside it (CONTRADICTION: NO toilet paper), as described in the caption (CAPTION: spare rolls of toilet paper)\\
\\
CAPTION: A cat is holding a frisbee in its mouth\\
FEEDBACKS: ["A dog is holding a frisbee in its mouth", "A dog is holding a frisbee in its mouth.", "A dog is holding a frisbee, not a cat"]
\\
MISALIGNMENT: \\

\midrule
Generation\\
\midrule
CAPTION: A cat is holding a frisbee in its mouth\\
FEEDBACKS: ["A dog is holding a frisbee in its mouth", "A dog is holding a frisbee in its mouth.", "A dog is holding a frisbee, not a cat"]\\
MISALIGNMENT: The animal holding the frisbee is a dog (CONTRADICTION: dog holding a frisbee), not a cat (CAPTION: cat holding a frisbee)\\
\bottomrule
\end{tabular}    
\caption{Few-shot prompt example for generating the required labels for our \testset test dataset from human-annotated feedbacks.}
\label{fig:prompt_seetrue}

\end{figure*}


==> preamble.tex <==
\RequirePackage[numbers,sort&compress, square, sort]{natbib}

\usepackage{natbib}
\usepackage{wrapfig}
% --- inline annotations
%
%\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


\newcommand{\danix}[1]{{\color{magenta}[\textbf{danix:} #1]}}
\newcommand{\dl}[1]{{\color{brown}#1}}
\newcommand{\dc}[1]{{\color{magenta}#1}}
\newcommand{\brian}[1]{{\color{orange}[\textbf{brian:} #1]}}
\newcommand{\yoni}[1]{{\color{blue}[\textbf{yoni:} #1]}}
\newcommand{\yb}[1]{{\color{purple}[\textbf{yb:} #1]}}

% \newcommand{\danix}[1]{}
% \newcommand{\dl}[1]{}
% \newcommand{\dc}[1]{}
% \newcommand{\brian}[1]{}
% \newcommand{\yoni}[1]{}
% \newcommand{\yb}[1]{}

% Names
\newcommand{\method}{ConGen-Feedback\xspace}
\newcommand{\model}{VNLI-Feedback\xspace}
\newcommand{\testset}{SeeTRUE-Feedback\xspace}
\newcommand{\trainset}{TV-Feedback\xspace}
\newcommand{\pali}{PaLI\xspace}

 \newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\promptfont}{\fontsize{5.4pt}{6pt}\selectfont}


\let\titleold\title
\renewcommand{\title}[1]{\titleold{#1}\newcommand{\thetitle}{#1}}
\def\maketitlesupplementary
   {
        \centering
        \Large
        \textbf{\thetitle}\\
        \vspace{0.5em}Supplementary Material \\
        \vspace{1.0em}
   }
\newif\ifAppendixEnable
\AppendixEnabletrue

==> prompts/imagereward_noun.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \begin{tabular}{p{\linewidth}}
    \toprule
Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models. \\
\\
Guidelines:\\
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. \\
The elucidation should:\\
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., ''CAPTION: a blue ball on a shelf'').\\
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., ''CONTRADICTION: green ball'').\\
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\

\\
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.\\
\\
Examples: \\
\\
CAPTION: a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background\\
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background\\
MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure \\standing on a rock (CAPTION: robotic action figure standing on a rock)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background\\
CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background\\
MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .\\
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .\\
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a painting of a landscape with mountains and clouds in the sky\\
CONTRADICTION: a painting of a landscape with a beach and clouds in the sky\\
MISALIGNMENT: The painting is of a landscape with mountains (CAPTION: landscape with mountains) , not trees (CONTRADICTION: landscape with a beach) .\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: A black and green cat figurine on a gray surface.\\
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.\\
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a black and white drawing of a person wearing a helmet and headphones\\
CONTRADICTION: a black and white drawing of a person wearing a helmet and sunglasses\\
MISALIGNMENT: The person is wearing a headphone (CAPTION: person wearing a helmet and headphones), not sunglasses (CONTRADICTION: person wearing a helmet and sunglasses).\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a silhouette of a person standing in a forest with a castle in the background\\
CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background\\
MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand\\
CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water\\
MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)\\
MISALIGNMENT TYPE: Object/Noun\\
         \\
        \bottomrule
    \end{tabular}
    
    \caption{\color{red}WIP: Few-shot prompt example. This prompt is used to generate an \textit{object} misalignment type on ImageReward~\cite{xu2023imagereward} dataset.}
\end{figure*}


==> prompts/imagereward_noun2.tex <==
The following figures illustrate the formatting and phrasing of all the tasks included in the paper. All data comes from the ground truth datasets in this section, and no samples from GPT-3 are included here.


\begin{figure*} {  \footnotesize \begin{tabularx}{\linewidth}{r X} \toprule 
Context $\to$ &  Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models. \\
 \\
 & Guidelines:\\
 & Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
 & MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. \\
 & The elucidation should:\\
 & Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
 & For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., CAPTION: ``a blue ball on a shelf'').\\
 & For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., CONTRADICTION: ``green ball'').\\
 & MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\
\midrule
Few-Shot $\to$ &  Guidelines: \\
 & - Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.\\
\\
 & Examples: \\
\\
 & CAPTION: a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background\\
 & CONTRADICTION: a woman standing on a rock in the desert with mountains in the background\\
 & MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure standing on a rock (CAPTION: robotic action figure standing on a rock)\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background\\
 & CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background\\
 & MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .\\
 & CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .\\
 & MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: a painting of a landscape with mountains and clouds in the sky\\
 & CONTRADICTION: a painting of a landscape with a beach and clouds in the sky\\
 & MISALIGNMENT: The painting is of a landscape with mountains (CAPTION: landscape with mountains) , not trees (CONTRADICTION: landscape with a beach) .\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: A black and green cat figurine on a gray surface.\\
 & CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.\\
 & MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: a black and white drawing of a person wearing a helmet and headphones\\
 & CONTRADICTION: a black and white drawing of a person wearing a helmet and sunglasses\\
 & MISALIGNMENT: The person is wearing a headphone (CAPTION: person wearing a helmet and headphones), not sunglasses (CONTRADICTION: person wearing a helmet and sunglasses).\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: a silhouette of a person standing in a forest with a castle in the background\\
 & CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background\\
 & MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)\\
 & MISALIGNMENT TYPE: Object/Noun\\
\\
 & CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand\\
 & CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water\\
 & MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)\\
 & MISALIGNMENT TYPE: Object/Noun \\
 \\
 & CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand \\
\midrule
Generated $\to$ & CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand \\
 & CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water\\
 & MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)\\
 & MISALIGNMENT TYPE: Object/Noun \\
 \bottomrule 
 \end{tabularx} }  
 \caption{{\color{red} TODO!}}  
 \label{eval:RACE-h}  
 \end{figure*}

==> prompts/imagereward_noun3.tex <==
\begin{figure*}
    \centering
    \footnotesize
    \begin{tabular}{p{\linewidth}}
    \toprule
Context\\
\midrule
Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models. \\
\\
Guidelines:\\
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.\\
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. \\
The elucidation should:\\
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.\\
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").\\
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").\\
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation\\
\midrule
Few-Shot \\
\midrule
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.\\
\\
Examples: \\
\\
CAPTION: a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background\\
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background\\
MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure \\standing on a rock (CAPTION: robotic action figure standing on a rock)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background\\
CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background\\
MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .\\
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .\\
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.\\
MISALIGNMENT TYPE: Object/Noun\\
 \\
CAPTION: a black and white drawing of a person wearing a helmet and headphones\\
CONTRADICTION: a black and white drawing of a person wearing a helmet and sunglasses\\
MISALIGNMENT: The person is wearing a headphone (CAPTION: person wearing a helmet and headphones), not sunglasses (CONTRADICTION: person wearing a helmet and sunglasses).\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a silhouette of a person standing in a forest with a castle in the background\\
CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background\\
MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand\\
CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water\\
MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)\\
MISALIGNMENT TYPE: Object/Noun\\
\\
Create a MISALIGNMENT of type: Object/Noun \\
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it. \\
CAPTION: A samurai in armor and a helmet is holding a sword against a sunset sky with clouds\\

\midrule
Generation\\
\midrule
CAPTION: A samurai in armor and a helmet is holding a sword against a sunset sky with clouds\\
CONTRADICTION: A samurai in armor and a helmet is holding a gun against a sunset sky with clouds\\
MISALIGNMENT: The samurai is holding a sword (CAPTION: sword), not a gun (CONTRADICTION: gun)\\
MISALIGNMENT TYPE: Object/Noun\\
\bottomrule
\end{tabular}    
    \caption{\color{red}WIP: Few-shot prompt example. This prompt is used to generate an \textit{object} misalignment type on ImageReward~\cite{xu2023imagereward} dataset.}
\end{figure*}


==> prompts/raw_prompts/coco.tex <==
OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A stained glass window with a cartoon image of a man with glasses and a beard .
CONTRADICTION: A stained glass window with a cartoon image of a man with a beard .
MISALIGNMENT: The man in stained glass wear glasses (CAPTION: man with glasses and a beard), instead of only beard (CONTRADICTION: man with a beard).
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A sign welcomes visitors to Lake Kawaguchiko in English and in another language.
CONTRADICTION: A mascot welcomes visitors to Lake Kawaguchiko in Japanese and in another language.
MISALIGNMENT: There is a sign welcoming visitors to Lake Kawaguchiko (CAPTION: sign), not a mascot (CONTRADICTION: mascot)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Two dogs on a leash playing on the shore and in the water of a lake.
CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano.
MISALIGNMENT: The dogs are playing on the shore and in the water of a lake (CAPTION: Two dogs on a leash playing on the shore and in the water of a lake), not a volcano (CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano).
MISALIGNMENT TYPE: Object/Noun

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Three pigeons on the side walk munching on a thrown out breadstick.
CONTRADICTION: Eight pigeons on the side walk munching on a thrown out pizza crust.
MISALIGNMENT: There are three pigeons eating a breadstick (CAPTION: Three pigeons munching on a breadstick), not eight. (CONTRADICTION: Eight pigeons munching on a breadstick)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A box of pizza with peppers, onions and sausage on it.
CONTRADICTION: A box of pizza with pineapple on it.
MISALIGNMENT: The pizza has peppers, onions and mushrooms on it (CAPTION: peppers, onions and mushrooms), not pineapple (CONTRADICTION: pineapple)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A baseball player holding a bat while standing next to a home plate.
CONTRADICTION: A baseball player holding a bat while standing next to Batman.
MISALIGNMENT: The baseball player is not holding a bat next to Batman (CONTRADICTION: player next to Batman) , instead is next to a home plate (CAPTION: player next to home plate) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A woman playing tennis is swinging at a tennis ball.
CONTRADICTION: A woman playing tennis is juggling tennis balls.
MISALIGNMENT: The woman is swinging at a tennis ball (CAPTION: woman playing tennis is swinging at a tennis ball), not juggling tennis balls (CONTRADICTION: woman playing tennis is juggling tennis balls).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A bird is sitting on a branch eating a banana peel.
CONTRADICTION: A bird is sitting on a branch eating an apple.
MISALIGNMENT: The bird is eating an apple (CAPTION: bird eating an apple), not a banana peel (CONTRADICTION: bird eating a banana peel).
MISALIGNMENT TYPE: Object/Noun
"""

ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"
CONTRADICTION: a cartoon of a mermaid with black hair in the water
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with black hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A cartoon drawing of a person with bat wings on a white paper with a keyboard and pens on a table ."
CONTRADICTION: A cartoon drawing of a person with angel wings on a white paper with a keyboard and pens on a table.
MISALIGNMENT: The person wings are bat wings (CAPTION: person with bat wings), not angel wings (CONTRADICTION: person with angle wings).
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a naked woman with long hair on a grey background
CONTRADICTION: A portrait of a naked woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: The colorful flowers are in the vase next to the window.
CONTRADICTION: The white and black flowers are in the vase next to the window.
MISALIGNMENT: The flowers are colorful (CAPTION: colorful flowers) , not white and black (CONTRADICTION: white and black flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: Vase sitting next to the window with droopy flowers in it.
CONTRADICTION: Vase sitting next to the window with fresh flowers in it.
MISALIGNMENT: The vase has droppy flowers (CAPTION: droppy flowers), not fresh flowers (CAPTION: fresh flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A bicycle chained to a red pole and a green pole on the sidewalk in front of a building.
CONTRADICTION: A bicycle chained to a red pole and a blue pole on the sidewalk in front of a building.
MISALIGNMENT: One of the poles is red (CAPTION: green pole), not blue (CONTRADICTION: blue pole)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a kid trying to use a skating board on the road
CONTRADICTION: a kid breaking a skating board on the road
MISALIGNMENT: The kid is trying to use a skating board (CAPTION: kid trying to use a skating board), not breaking it (CONTRADICTION: kid breaking a skating board)
MISALIGNMENT TYPE: Action/Verb

CAPTION: Seated person wearing blue jeans holding a white corded electronic device.
CONTRADICTION: Seated person wearing blue jeans chewing a white cordless electronic device.
MISALIGNMENT: The person is holding a corded electronic device (CAPTION: person holding a white corded electronic device), not chewing a corded electronic device (CONTRADICTION: person chewing a corded electronic device)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A cup, saucer and spoon sitting next to a newspaper.
CONTRADICTION: A cup, saucer, and spoon flying next to a newspaper.
MISALIGNMENT: The cup, saucer, and spoon are sitting (CAPTION: cup, saucer, and spoon sitting next to a newspaper), not flying (CONTRADICTION: cup, saucer, and spoon flying next to a newspaper).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A man that is standing in the grass with a kite.
Contradiction: A man that is lying in the grass with a kite.
Misalignment: The man is standing (CAPTION: man standing in the grass with a kite), not lying (CONTRADICTION: man lying in the grass with a kite).
Misalignment Type: Action/Verb

"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation

CAPTION: Old fashioned chests are stacked atop each other on a city block.
CONTRADICTION: Old fashioned chests are stacked next to each other on a city block.
MISALIGNMENT: The chests are stacked atop each other (CAPTION: chests stacked atop each other), not next to each other (CONTRADICTION: chests stacked next to each other).
MISALIGNMENT TYPE: Relation

CAPTION: Boy holding large stuffed toy bear outside of building.
CONTRADICTION: Boy holding large stuffed toy bear inside of building.
MISALIGNMENT: The boy is outside of a building (CAPTION: Boy holding large stuffed toy bear outside of building), not inside of it  (CONTRADICTION: boy holding large stuffed toy bear inside of building) .
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation
"""

CONGEN_SAMPLE = """Create a MISALIGNMENT of type: <misalignment_type>
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.
CAPTION: <context_captions>
"""


==> prompts/raw_prompts/flickr30k.tex <==
BASE_CONGEN_PROMPT_V3_MERGED_MISALIGNMENT = """Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.

Guidelines:
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation
"""

OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A stained glass window with a cartoon image of a man with glasses and a beard .
CONTRADICTION: A stained glass window with a cartoon image of a man with a beard .
MISALIGNMENT: The man in stained glass wear glasses (CAPTION: man with glasses and a beard), instead of only beard (CONTRADICTION: man with a beard).
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A sign welcomes visitors to Lake Kawaguchiko in English and in another language.
CONTRADICTION: A mascot welcomes visitors to Lake Kawaguchiko in Japanese and in another language.
MISALIGNMENT: There is a sign welcoming visitors to Lake Kawaguchiko (CAPTION: sign), not a mascot (CONTRADICTION: mascot)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Two dogs on a leash playing on the shore and in the water of a lake.
CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano.
MISALIGNMENT: The dogs are playing on the shore and in the water of a lake (CAPTION: Two dogs on a leash playing on the shore and in the water of a lake), not a volcano (CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano).
MISALIGNMENT TYPE: Object/Noun

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Three pigeons on the side walk munching on a thrown out breadstick.
CONTRADICTION: Eight pigeons on the side walk munching on a thrown out pizza crust.
MISALIGNMENT: There are three pigeons eating a breadstick (CAPTION: Three pigeons munching on a breadstick), not eight. (CONTRADICTION: Eight pigeons munching on a breadstick)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A box of pizza with peppers, onions and sausage on it.
CONTRADICTION: A box of pizza with pineapple on it.
MISALIGNMENT: The pizza has peppers, onions and mushrooms on it (CAPTION: peppers, onions and mushrooms), not pineapple (CONTRADICTION: pineapple)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A baseball player holding a bat while standing next to a home plate.
CONTRADICTION: A baseball player holding a bat while standing next to Batman.
MISALIGNMENT: The baseball player is not holding a bat next to Batman (CONTRADICTION: player next to Batman) , instead is next to a home plate (CAPTION: player next to home plate) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A woman playing tennis is swinging at a tennis ball.
CONTRADICTION: A woman playing tennis is juggling tennis balls.
MISALIGNMENT: The woman is swinging at a tennis ball (CAPTION: woman playing tennis is swinging at a tennis ball), not juggling tennis balls (CONTRADICTION: woman playing tennis is juggling tennis balls).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A bird is sitting on a branch eating a banana peel.
CONTRADICTION: A bird is sitting on a branch eating an apple.
MISALIGNMENT: The bird is eating an apple (CAPTION: bird eating an apple), not a banana peel (CONTRADICTION: bird eating a banana peel).
MISALIGNMENT TYPE: Object/Noun
"""


ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"
CONTRADICTION: a cartoon of a mermaid with black hair in the water
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with black hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A cartoon drawing of a person with bat wings on a white paper with a keyboard and pens on a table ."
CONTRADICTION: A cartoon drawing of a person with angel wings on a white paper with a keyboard and pens on a table.
MISALIGNMENT: The person wings are bat wings (CAPTION: person with bat wings), not angel wings (CONTRADICTION: person with angle wings).
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a naked woman with long hair on a grey background
CONTRADICTION: A portrait of a naked woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: The colorful flowers are in the vase next to the window.
CONTRADICTION: The white and black flowers are in the vase next to the window.
MISALIGNMENT: The flowers are colorful (CAPTION: colorful flowers) , not white and black (CONTRADICTION: white and black flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: Vase sitting next to the window with droopy flowers in it.
CONTRADICTION: Vase sitting next to the window with fresh flowers in it.
MISALIGNMENT: The vase has droppy flowers (CAPTION: droppy flowers), not fresh flowers (CAPTION: fresh flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A bicycle chained to a red pole and a green pole on the sidewalk in front of a building.
CONTRADICTION: A bicycle chained to a red pole and a blue pole on the sidewalk in front of a building.
MISALIGNMENT: One of the poles is red (CAPTION: green pole), not blue (CONTRADICTION: blue pole)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a kid trying to use a skating board on the road
CONTRADICTION: a kid breaking a skating board on the road
MISALIGNMENT: The kid is trying to use a skating board (CAPTION: kid trying to use a skating board), not breaking it (CONTRADICTION: kid breaking a skating board)
MISALIGNMENT TYPE: Action/Verb

CAPTION: Seated person wearing blue jeans holding a white corded electronic device.
CONTRADICTION: Seated person wearing blue jeans chewing a white cordless electronic device.
MISALIGNMENT: The person is holding a corded electronic device (CAPTION: person holding a white corded electronic device), not chewing a corded electronic device (CONTRADICTION: person chewing a corded electronic device)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A cup, saucer and spoon sitting next to a newspaper.
CONTRADICTION: A cup, saucer, and spoon flying next to a newspaper.
MISALIGNMENT: The cup, saucer, and spoon are sitting (CAPTION: cup, saucer, and spoon sitting next to a newspaper), not flying (CONTRADICTION: cup, saucer, and spoon flying next to a newspaper).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A man that is standing in the grass with a kite.
CONTRADICTION: A man that is lying in the grass with a kite.
MISALIGNMENT: The man is standing (CAPTION: man standing in the grass with a kite), not lying (CONTRADICTION: man lying in the grass with a kite).
MISALIGNMENT TYPE: Action/Verb

CAPTION: a man sleeping on a bench outside with a white and black dog sitting next to him .
CONTRADICTION: a man sleeping on a bench outside with a white and black dog running next to him .
MISALIGNMENT: The dog is running (CAPTION: dog running), not sitting (CONTRADICTION: dog sitting)
MISALIGNMENT TYPE: Action/Verb
"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation

CAPTION: Old fashioned chests are stacked atop each other on a city block.
CONTRADICTION: Old fashioned chests are stacked next to each other on a city block.
MISALIGNMENT: The chests are stacked atop each other (CAPTION: chests stacked atop each other), not next to each other (CONTRADICTION: chests stacked next to each other).
MISALIGNMENT TYPE: Relation

CAPTION: Boy holding large stuffed toy bear outside of building.
CONTRADICTION: Boy holding large stuffed toy bear inside of building.
MISALIGNMENT: The boy is outside of a building (CAPTION: Boy holding large stuffed toy bear outside of building), not inside of it  (CONTRADICTION: boy holding large stuffed toy bear inside of building) .
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation
"""


==> prompts/raw_prompts/imagereward.tex <==
BASE_CONGEN_PROMPT_V3_MERGED_MISALIGNMENT = """Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.

Guidelines:
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation
"""

OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure standing on a rock (CAPTION: robotic action figure standing on a rock)
MISALIGNMENT TYPE: Object/Noun

CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background
CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background
MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: a painting of a landscape with mountains and clouds in the sky
CONTRADICTION: a painting of a landscape with a beach and clouds in the sky
MISALIGNMENT: The painting is of a landscape with mountains (CAPTION: landscape with mountains) , not trees (CONTRADICTION: landscape with a beach) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: a black and white drawing of a person wearing a helmet and headphones
CONTRADICTION: a black and white drawing of a person wearing a helmet and sunglasses
MISALIGNMENT: The person is wearing a headphone (CAPTION: person wearing a helmet and headphones), not sunglasses (CONTRADICTION: person wearing a helmet and sunglasses).
MISALIGNMENT TYPE: Object/Noun

CAPTION: a silhouette of a person standing in a forest with a castle in the background
CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background
MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)
MISALIGNMENT TYPE: Object/Noun

CAPTION: a black and white landscape of an iceberg in the ocean with a boat on the sand
CONTRADICTION: a black and white landscape of an iceberg in the ocean with a boat in the water
MISALIGNMENT: The boat is in the sand (CAPTION: boat on the sand), not on the sand (CONTRADICTION: boat in the water)
MISALIGNMENT TYPE: Object/Noun
"""

ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: a gold coin with a logo on it on a gray wall
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a waterfall in a tropical forest with green plants and trees
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A cartoon drawing of a person with bat wings on a white paper with a keyboard and pens on a table .
CONTRADICTION: A cartoon drawing of a person with angel wings on a white paper with a keyboard and pens on a table.
MISALIGNMENT: The person wings are bat wings (CAPTION: person with bat wings), not angel wings (CONTRADICTION: person with angle wings).
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a woman with long hair on a grey background
CONTRADICTION: A portrait of a woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A futuristic spider toy and a robotic spider toy on a gray surface .
CONTRADICTION: A futuristic spider toy and a plastic spider toy on a gray surface
MISALIGNMENT: The spider toy is robotic (CONTRADICTION: robotic spider toy), not plastic (CAPTION: plastic spider toy)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a black and white drawing of a light fixture with a gray background
CONTRADICTION: A colorful drawing of a light fixture with a gray background
MISALIGNMENT: The drawing is not colorful (CONTRADICTION: colorful drawing) , instead is black and white (CAPTION: black and white drawing) .
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a painting of a skeleton person with a skull face and a hooded person with a skull face
CONTRADICTION: A painting of a real person with a skull face and a hooded person with a skull face
MISALIGNMENT: The person is not real (CONTRADICTION: real person), but a skeleton (CAPTION: skeleton person)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A black and white portrait of a bald man with glasses and a beard .
CONTRADICTION: A black and white portrait of a bald man with glasses and an eyepatch
MISALIGNMENT: The man has glasses and beard (CONTRADICTION: man with glasses and a beard), not glasses and eyepatch (CAPTION: man with glasses and an eyepatch) .
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a red color smoke coming from a fire in the sky with clouds and grass on the ground
CONTRADICTION: a blue color smoke coming from a fire in the sky with clouds and grass on the ground
MISALIGNMENT: The smoke is red (CAPTION: red color smoke), not blue (CONTRADICTION: blue color smoke)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane drinking water on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion drinking water)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A cartoon of a man in a suit and hat sitting at a table in a city with buildings and a blue sky."
CONTRADICTION: A cartoon of a man in a suit and hat jumping on a table in a city with buildings and a blue sky.
MISALIGNMENT: The man is not jumping (CONTRADICTION: man in a suit and hat jumping) , instead is sitting at the table (CAPTION: man in a suit and hat sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a futuristic spaceship flying in the sky with clouds and stars in the background
CONTRADICTION: a futuristic spaceship explodes in the sky with clouds and stars in the background
MISALIGNMENT: The spaceship is not exploded (CONTRADICTION: spaceship explodes), instead is flying (CAPTION: spaceship flying)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a fantasy painting of a forest with a river flowing through it and trees in the background
"CONTRADICTION: a fantasy painting of a forest with a river freeze through it and trees in the background
MISALIGNMENT: The river is flowing (CONTRADICTION: river flowing), not freeze (CAPTION: river freeze)
MISALIGNMENT TYPE: Action/Verb"
"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: a black and white drawing of a light fixture with a gray background
CONTRADICTION: A colorful drawing of a light fixture with a gray background
MISALIGNMENT: The drawing is not colorful (CONTRADICTION: colorful drawing) , instead is black and white (CAPTION: black and white drawing) .
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: a futuristic spaceship flying in the sky with clouds and stars in the background
CONTRADICTION: a futuristic spaceship explodes in the sky with clouds and stars in the background
MISALIGNMENT: The spaceship is not exploded (CONTRADICTION: spaceship explodes), instead is flying (CAPTION: spaceship flying)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a silhouette of a person standing in a forest with a castle in the background
CONTRADICTION: a silhouette of a dragon standing in a forest with a city in the background
MISALIGNMENT: The silhouette is of a person (CAPTION: silhouette of a person), not a dragon (CONTRADICTION: silhouette of a dragon)
MISALIGNMENT TYPE: Object/Noun
"""


==> prompts/raw_prompts/localized_narratives.tex <==
BASE_CONGEN_PROMPT_V3_MERGED_MISALIGNMENT = """Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.

Guidelines:
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation
"""

OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A sign welcomes visitors to Lake Kawaguchiko in English and in another language.
CONTRADICTION: A mascot welcomes visitors to Lake Kawaguchiko in Japanese and in another language.
MISALIGNMENT: There is a sign welcoming visitors to Lake Kawaguchiko (CAPTION: sign), not a mascot (CONTRADICTION: mascot)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Two dogs on a leash playing on the shore and in the water of a lake.
CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano.
MISALIGNMENT: The dogs are playing on the shore and in the water of a lake (CAPTION: Two dogs on a leash playing on the shore and in the water of a lake), not a volcano (CONTRADICTION: Two dogs on a leash playing on the shore and in the water of a volcano).
MISALIGNMENT TYPE: Object/Noun

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: Three pigeons on the side walk munching on a thrown out breadstick.
CONTRADICTION: Eight pigeons on the side walk munching on a thrown out pizza crust.
MISALIGNMENT: There are three pigeons eating a breadstick (CAPTION: Three pigeons munching on a breadstick), not eight. (CONTRADICTION: Eight pigeons munching on a breadstick)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A box of pizza with peppers, onions and sausage on it.
CONTRADICTION: A box of pizza with pineapple on it.
MISALIGNMENT: The pizza has peppers, onions and mushrooms on it (CAPTION: peppers, onions and mushrooms), not pineapple (CONTRADICTION: pineapple)
MISALIGNMENT TYPE: Object/Noun

CAPTION: A baseball player holding a bat while standing next to a home plate.
CONTRADICTION: A baseball player holding a bat while standing next to Batman.
MISALIGNMENT: The baseball player is not holding a bat next to Batman (CONTRADICTION: player next to Batman) , instead is next to a home plate (CAPTION: player next to home plate) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A woman playing tennis is swinging at a tennis ball.
CONTRADICTION: A woman playing tennis is juggling tennis balls.
MISALIGNMENT: The woman is swinging at a tennis ball (CAPTION: woman playing tennis is swinging at a tennis ball), not juggling tennis balls (CONTRADICTION: woman playing tennis is juggling tennis balls).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A bird is sitting on a branch eating a banana peel.
CONTRADICTION: A bird is sitting on a branch eating an apple.
MISALIGNMENT: The bird is eating an apple (CAPTION: bird eating an apple), not a banana peel (CONTRADICTION: bird eating a banana peel).
MISALIGNMENT TYPE: Object/Noun

CAPTION: A room with a chandelier, chairs and pillars.
CONTRADICTION: A room with a fountain, chairs and a table.
MISALIGNMENT: The room has a chandelier (CAPTION: a chandelier) , instead of a fountain (CONTRADICTION: a fountain) .
MISALIGNMENT TYPE: Object/Noun

CAPTION: A view of a mountain range with grass, plants, and trees.
CONTRADICTION: A view of a mountain range with grass, plants, and a lake.
MISALIGNMENT: There are grass, plants and trees in the view (CAPTION: mountain range with grass, plants, and trees) , no lake (CONTRADICTION: mountain range with grass, plants, and a lake.)
MISALIGNMENT TYPE: Object/Noun
"""


ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"
CONTRADICTION: a cartoon of a mermaid with black hair in the water
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with black hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a naked woman with long hair on a grey background
CONTRADICTION: A portrait of a naked woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: The colorful flowers are in the vase next to the window.
CONTRADICTION: The white and black flowers are in the vase next to the window.
MISALIGNMENT: The flowers are colorful (CAPTION: colorful flowers) , not white and black (CONTRADICTION: white and black flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: Vase sitting next to the window with droopy flowers in it.
CONTRADICTION: Vase sitting next to the window with fresh flowers in it.
MISALIGNMENT: The vase has droppy flowers (CAPTION: droppy flowers), not fresh flowers (CAPTION: fresh flowers)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: A bicycle chained to a red pole and a green pole on the sidewalk in front of a building.
CONTRADICTION: A bicycle chained to a red pole and a blue pole on the sidewalk in front of a building.
MISALIGNMENT: One of the poles is red (CAPTION: green pole), not blue (CONTRADICTION: blue pole)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a kid trying to use a skating board on the road
CONTRADICTION: a kid breaking a skating board on the road
MISALIGNMENT: The kid is trying to use a skating board (CAPTION: kid trying to use a skating board), not breaking it (CONTRADICTION: kid breaking a skating board)
MISALIGNMENT TYPE: Action/Verb

CAPTION: Seated person wearing blue jeans holding a white corded electronic device.
CONTRADICTION: Seated person wearing blue jeans chewing a white cordless electronic device.
MISALIGNMENT: The person is holding a corded electronic device (CAPTION: person holding a white corded electronic device), not chewing a corded electronic device (CONTRADICTION: person chewing a corded electronic device)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A cup, saucer and spoon sitting next to a newspaper.
CONTRADICTION: A cup, saucer, and spoon flying next to a newspaper.
MISALIGNMENT: The cup, saucer, and spoon are sitting (CAPTION: cup, saucer, and spoon sitting next to a newspaper), not flying (CONTRADICTION: cup, saucer, and spoon flying next to a newspaper).
MISALIGNMENT TYPE: Action/Verb

CAPTION: A man that is standing in the grass with a kite.
Contradiction: A man that is lying in the grass with a kite.
Misalignment: The man is standing (CAPTION: man standing in the grass with a kite), not lying (CONTRADICTION: man lying in the grass with a kite).
Misalignment Type: Action/Verb

CAPTION: A woman stands while people sit at a table.
CONTRADICTION: A woman sits while people stand at a table.
MISALIGNMENT: The woman is standing (CAPTION: woman stands), not sitting (CONTRADICTION: woman sits)
MISALIGNMENT TYPE: Action/Verb
"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation

CAPTION: Old fashioned chests are stacked atop each other on a city block.
CONTRADICTION: Old fashioned chests are stacked next to each other on a city block.
MISALIGNMENT: The chests are stacked atop each other (CAPTION: chests stacked atop each other), not next to each other (CONTRADICTION: chests stacked next to each other).
MISALIGNMENT TYPE: Relation

CAPTION: Boy holding large stuffed toy bear outside of building.
CONTRADICTION: Boy holding large stuffed toy bear inside of building.
MISALIGNMENT: The boy is outside of a building (CAPTION: Boy holding large stuffed toy bear outside of building), not inside of it  (CONTRADICTION: boy holding large stuffed toy bear inside of building) .
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: a man kneeling on a surfboard as he starts to ride a wave
CONTRADICTION: a man hand-standing on a surfboard as he starts to ride a wave 
MISALIGNMENT: The surfer is kneeling on a surfboard (CAPTION: a man kneeling on a surfboard), not performing a hand-standing on it. (CONTRADICTION: a man hand-standing on a surfboard)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation
"""


CONGEN_SAMPLE = """Create a MISALIGNMENT of type: <misalignment_type>
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.
CAPTION: <context_captions>
"""

==> prompts/raw_prompts/pickapic.tex <==
BASE_CONGEN_PROMPT_V3_MERGED_MISALIGNMENT = """Your primary task is to generate subtly contradictory captions based on an original input caption. This test is intended to observe the capacity of models to recognize nuanced semantic changes which might be easily detected by humans but challenging for models.

Guidelines:
Caption Modification: Introduce a delicate semantic change to the original caption. The alteration should subtly change the meaning while remaining potentially overlooked. It should neither be drastic nor too minor.
MISALIGNMENT: After constructing your contradictory caption, articulate the disparity between the original CAPTION and the CONTRADICTION in a crisp manner. The elucidation should:
Spotlight the deviation from the angle of the CONTRADICTION, pinpointing what the CONTRADICTION suggests but is countered by the CAPTION.
For the CAPTION description, ensure it thoroughly represents the true content of the CAPTION (e.g., "CAPTION: a blue ball on a shelf").
For the CONTRADICTION description, keep it brief and directly replicate the relevant segment (e.g., "CONTRADICTION: green ball").
MISALIGNMENT TYPE: Categorize the nature of the misalignment into one of the following categories: Object/Noun, Attribute/Adjective, Action/Verb, or Relation
"""

OBJECT_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Object/Noun Misalignment: Change a key object or noun in the caption to create a contradiction, you can also add or remove an object, or alter the quantity of an item. The contradictory caption should then focus on a different object/noun, and this discrepancy must be clearly highlighted in the misalignment description.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: woman), instead there is a robotic action figure standing on a rock (CAPTION: robotic action figure standing on a rock)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a painting of a ballroom with a chandelier hanging from the ceiling and two persons standing on the floor"
CONTRADICTION: a painting of a bedroom with a chandelier hanging from the ceiling and two persons standing on the floor
MISALIGNMENT: The scene is of a ballroom (CAPTION: ballroom with a chandelier), not a bedroom (CONTRADICTION: bedroom)
MISALIGNMENT TYPE: Object/Noun

CAPTION: portrait of a beautiful woman with short hair in a white t shirt on the street with trees in the background
CONTRADICTION: portrait of a beautiful alien with short hair in a white t shirt on the street with trees in the background
MISALIGNMENT: A woman (CAPTION: woman) , not an alien  (CONTRADICTION: alien) , is the subject of the portrait.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A cartoon painting of three cats and a mouse on a yellow wall .
CONTRADICTION: A cartoon painting of five cats and a mouse on a yellow wall .
MISALIGNMENT: Three cats (CAPTION: three cats), not five are in the cartoon painting.
MISALIGNMENT TYPE: Object/Noun

CAPTION: A stained glass window with a cartoon image of a man with glasses and a beard .
CONTRADICTION: A stained glass window with a cartoon image of a man with a beard .
MISALIGNMENT: The man in stained glass wear glasses (CAPTION: man with glasses and a beard), instead of only beard (CONTRADICTION: man with a beard).
MISALIGNMENT TYPE: Object/Noun

CAPTION: A black and green cat figurine on a gray surface.
CONTRADICTION: A black and green cat with a funny unicorn figurine on a gray surface.
MISALIGNMENT: The funny unicorn (CONTRADICTION: funny unicorn) is missing (CAPTION: None:) .
MISALIGNMENT TYPE: Object/Noun
"""

ATTR_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Attribute/Adjective Misalignment: Alter an attribute or adjective that describes an object or scene in the original caption. This alteration should create a contradiction in the description. Ensure that the changed attribute/adjective remains plausible within the context of the caption and doesn't alter the core meaning. The discrepancy between the original caption's attribute and the contradictory attribute should be highlighted in the misalignment description.

Examples: 

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a cartoon of a red haired mermaid holding a fish in the sea"
CONTRADICTION: a cartoon of a mermaid with long black hair in the water
MISALIGNMENT: The hair of the cartoon mermaid is red (CAPTION: red haired mermaid), not black (CONTRADICTION: mermaid with long black hair)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A cartoon drawing of a person with bat wings on a white paper with a keyboard and pens on a table ."
CONTRADICTION: A cartoon drawing of a person with angel wings on a white paper with a keyboard and pens on a table.
MISALIGNMENT: The person wings are bat wings (CAPTION: person with bat wings), not angel wings (CONTRADICTION: person with angle wings).
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: portrait of a woman with long hair on a grey background
CONTRADICTION: A portrait of a woman with short hair on a grey background
MISALIGNMENT: The woman has long hair (CAPTION: long hair), not short hair (CONTRADICTION: short hair)
MISALIGNMENT TYPE: Attribute/Adjective
"""

VERB_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Action/Verb Misalignment: Modify a central action or verb in the original caption. This change should introduce a contradiction in terms of the activity or behavior described. The changed verb should make sense within the context and should neither be too drastic nor too obscure. Ensure the difference between the original caption's action and the contradictory action is clearly and succinctly articulated in the misalignment description.

Examples: 

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane drinking water on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion drinking water)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A painting of a man standing in front of a fire in a field with trees and sky in the background ."
CONTRADICTION: A painting of a man running in front of a fire in a field with trees and a cloudy sky .
MISALIGNMENT: The main the painting is standing (CAPTION: man standing in front of a fire), not running (CONTRADICTION: man running in front of a fire)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A cartoon of a man in a suit and hat sitting at a table in a city with buildings and a blue sky."
CONTRADICTION: A cartoon of a man in a suit and hat jumping on a table in a city with buildings and a blue sky.
MISALIGNMENT: The man is not jumping (CONTRADICTION: man in a suit and hat jumping) , instead is sitting at the table (CAPTION: man in a suit and hat sitting)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A tattooed woman in a purple brassiere and purple underpants is standing in front of a table with a bottle on it."
CONTRADICTION: A tattooed woman in a purple brassiere and purple underpants is dancing in front of a table with a bottle on it.
MISALIGNMENT: The woman is not dancing (CONTRADICTION: tattooed woman dancing), instead is sitting (CAPTION: A tattooed woman is standing)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "portrait of a smiling man and woman hugging each other on the street with trees and buildings in the backgroun"
CONTRADICTION: portrait of a smiling man and woman fighting on the street with trees and buildings in the background
MISALIGNMENT: The man and woman are not fighting each other (CONTRADICTION: man and woman fighting), instead are hugging (CAPTION: a smiling man and woman hugging each other)
MISALIGNMENT TYPE: Action/Verb

CAPTION: A black background with a picture of a guy in a red hat jumping with a skate board.
CONTRADICTION: A black background with a picture of a guy in a red hat drinking water with a skate board.
MISALIGNMENT: The guy is not drinking water (CONTRADICTION: guy drinking water), instead is sitting (CAPTION: guy sitting)
MISALIGNMENT TYPE: Action/Verb
"""

RELATION_CONGEN_FEW_SHOT_PROMPT = """
Guidelines:
- Relation Misalignment: Change the relationship or position between objects. This entails tweaking prepositions, positioning, or context which defines the relationship between the mentioned items. In the misalignment description, specifically indicate the changed relation and the affected subjects.- Mention at the SOURCE fields the changed preposition and related subject

Examples: 

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch (CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation

CAPTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa near a gray wall
CONTRADICTION: portrait of a redhead girl with blue eyes in a violet color t shirt sitting on a yellow color sofa apart from a gray wall
MISALIGNMENT: The sofa is near the wall (CAPTION: a yellow sofa near a gray wall), not apart from it (CONTRADICTION: a yellow sofa apart from a gray wall)
MISALIGNMENT TYPE: Relation
"""

GENERAL_CONGEN_FEW_SHOT_PROMPT = """
Choose randomly from one of this misalignment types options :
- Object/Noun Misalignment: Change a key object or noun.
- Attribute/Adjective Misalignment: Modify an attribute of an object.
- Action/Verb Misalignment: Alter a specific action or verb performed by the object.
- Relation Misalignment: Change the relationship or position between objects.
Highlight Change: Explicitly mention what was changed between the CAPTION and the CONTRADICTION in the MISALIGNMENT section.

Examples: 

CAPTION: "a cartoon of a robotic action figure standing on a rock in the desert with mountains in the background"
CONTRADICTION: a woman standing on a rock in the desert with mountains in the background
MISALIGNMENT: No woman (CONTRADICTION: a woman standing on a rock), instead there is a robotic action (CAPTION: a cartoon of a robotic action figure standing on a rock) 
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a black and white image of a dark tunnel with a light shining through it"
CONTRADICTION: A black and white image of a dark mountain
MISALIGNMENT: This is a tunnel (CAPTION: a dark tunnel), not a black and white mountain (CONTRADICTION: dark mountain)
MISALIGNMENT TYPE: Object/Noun

CAPTION: "a gold coin with a logo on it on a gray wall"
CONTRADICTION: A gold coin with a logo on it is on an orange wall
MISALIGNMENT: The gold coin is on a gray wall (CAPTION: gray wall), not an orange wall (CONTRADICTION: orange wall)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "a waterfall in a tropical forest with green plants and trees"
CONTRADICTION: a waterfall in a snowy forest with green plants and trees
MISALIGNMENT: The forest is not snowy (CONTRADICTION: snowy forest), instead is a tropical one (CAPTION: tropical forest)
MISALIGNMENT TYPE: Attribute/Adjective

CAPTION: "A person dressed as Captain America is holding a shield in front of a wall."
CONTRADICTION: A person dressed as Captain America is throwing a shield and standing in front of a wall.
MISALIGNMENT: The person is not throwing a shield (CONTRADICTION: person throwing a shield), instead is holding it (CAPTION: person holding a shield)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "a close up of a lion with a long mane sitting on the grass with trees in the background"
CONTRADICTION: a close up of a lion with a long mane jumping on the grass in the forest with trees in the background
MISALIGNMENT: The lion is sitting (CAPTION: a lion sitting), not jumping on the grass (CONTRADICTION: lion jumping)
MISALIGNMENT TYPE: Action/Verb

CAPTION: "A laptop next to a stack of books on a wooden desk"
CONTRADICTION: A laptop under a stack of books on a wooden desk.
MISALIGNMENT: The laptop is next to the the books (CAPTION: laptop next to a stack of books), not under them (CONTRADICTION: laptop under a stack of books).
MISALIGNMENT TYPE: Relation

CAPTION: Two cats are sitting below a branch of a tree in front of a building with windows and trees in the background .
CONTRADICTION: Two cats are sitting above a branch of a tree in front of a building with windows and trees in the background .
MISALIGNMENT: The cats are in front of the building sitting below a branch(CAPTION: Two cats sitting below a branch), not above it (CONTRADICTION: Two cats sitting above a branch)
MISALIGNMENT TYPE: Relation
"""

CONGEN_SAMPLE = """Create a MISALIGNMENT of type: <misalignment_type>
Remember when writing the MISALIGNMENT that the expectation is that CONTRADICTION should happen, but instead we got the scene of CAPTION. We expect for CONTRADICTION but CAPTION counters it.
CAPTION: <context_captions>
"""


==> prompts/raw_prompts/seetrue.tex <==
BASE_CONGEN_PROMPT = """Your primary task is to generate a single summarized feedback based on visual feedback provided in the input, and identify the source of misalignment between the caption and the visual content. The goal is to extract meaningful insights from the feedback and link them to the corresponding elements in the caption.

Guidelines:
SUMMARIZED FEEDBACK: Given a caption and a set of visual feedbacks, your objective is to create a concise and informative feedback statement that captures the most significant misalignment between the caption and the visual content. No need to mention "at the caption" or "at the image".
Misalignment Identification: After constructing the summarized feedback, you should indicate the source of misalignment for both the caption and the visual content. In parentheses, specify the origin of the misalignment as follows:
CAPTION: Describe the source of misalignment that originates from the text (e.g., a description or detail in the caption that does not match the image). Mention also the related subject.
CONTRADICTION: Based on the feedback, pinpoint the source of misalignment in the visual content that contradicts the caption. Make sure the CONTRADICTION referes only to the relative part in FEEDBACKS. Mention also the related subject.


Examples:

CAPTION: "A woman with a blue shirt and yellow flower headband, sitting on a wooden bench outside on the grass."
FEEDBACKS: ["The woman's shirt is yellow, not blue.", "The woman sitting on the wooden bench is wearing a white shirt, not a blue shirt.", "The woman has a yellow shirt on, not blue."]
MISALIGNMENT: The sitting woman is wearing a yellow shirt (CONTRADICTION: yellow shirt), not a blue shirt (CAPTION: blue shirt)

CAPTION: "A banana on the left of an apple."
FEEDBACKS: ["The banana is to the right of the apple, not to its left.", "A banana on the right of an apple, not the left.", "The apple is to the left of a yellow pepper, but there is not a banana to the left of the apple"]
MISALIGNMENT: The banana is not on the left of the apple (CAPTION: banana left of an apple), instead it's on the right (CONTRADICTION: banana right of the apple)

CAPTION: "A donkey and an octopus are playing a game. The donkey is holding a rope on one end, the octopus is holding onto the other. The donkey holds the rope in its mouth. A cat is jumping over the rope."
FEEDBACKS: ["An octopus jumped over the rope, not a cat.", NaN, "There are three creatures, but no octopus or donkey"]
MISALIGNMENT: There are three creatures (CONTRADICTION: three creatures), but no donkey, octopus and cat (CAPTION: A donkey and an octopus. cat jumping rope).

CAPTION: A couch on the left of a chair.
FEEDBACKS: ["A couch is to the left of a coffee table, there is no chair present.", "A couch and two tables under a window, there is no chair.", NaN]
MISALIGNMENT: The couch is to the left of a table (CONTRADICTION: coffe table), not left of a chair (CAPTION: chair).

CAPTION: A sheep to the right of a wine glass.
FEEDBACKS: ["A sheep is facing the camera, not to the right of a wine glass, which is not present.", "A sheep looking at the camera, there is no wine glass.", "There is only a sheep alone in a field, it is not to the right of a wine glass"]
MISALIGNMENT: There is no wine glass (CAPTION: wine glass) (CONTRADICTION: no wine glass)

CAPTION: A tomato has been put on top of a pumpkin on a kitchen stool. There is a fork sticking into the pumpkin. The scene is viewed from above.
FEEDBACKS: [NaN, "A pumpkin has been put on top of a kitchen stool. There is a fork sticking into the pumpkin. The scene is viewed from above. There is no tomato on top of the pumpkin.", "There is only a pumpkin, and no tomato"]
MISALIGNMENT: There is no tomato on top of a pumpkin (CAPTION: tomato on top of a pumpkin) (CONTRADICTION: no tomato)

CAPTION: a red glass ball with a reflection on top of a gray surface
FEEDBACKS: ["The glass ball is blue, not red.", "The ball with the reflection should be blue instead of red.", "The ball is blue, not red"]
MISALIGNMENT: The color of the ball is blue (CONTRADICTION: blue ball), not red (CAPTION: red ball)

CAPTION: A lunch salad in a yellow bowl made out of fruit, vegetables, and meats with chopsticks. 
FEEDBACKS: ["There is no meat present, nor are there any chopsticks, simply the bowl with fruit and vegetable.", "There is a bowl of food, but no chopsticks.", "There is a salad with fruit and vegetables in a yellow bowl but there does not appear to be meat in it and there are no chopsticks."]
MISALIGNMENT: There is a yellow bowl with fruit and vegetables (CONTRADICTION: salad with fruit and vegetables in a yellow bowl) but without meat, also no chopsticks present (CAPTION: salad made out of fruit, vegetables, and meats with chopsticks)

CAPTION: A cup filled with umbrellas and canes next to a white wall.
FEEDBACKS: ["The wall is gray, not white.", "A bucket has two canes in it, not umbrellas and canes and it is front of a gray wall, not a white wall.", "A cup has canes in it, but no umbrellas"]
MISALIGNMENT: The cup has canes in it (CAPTION: umbrellas and canes), but no umbrellas (CONTRADICTION: no umbrellas). The wall is not white (CAPTION: white tall), instead is gray (CONTRADICTION: gray wall).

CAPTION: Small white toilet with spare rolls of toilet paper beside it.
FEEDBACKS:["A small white toilet is here without any rolls of toilet paper, not any spares.", "There is a toilet but no toilet paper.", "The toilet only has curtains/walls next to it, not spare rolls of toilet paper."]
MISALIGNMENT: The toilet does not have any spare rolls of toilet paper beside it (CONTRADICTION: NO toilet paper), as described in the caption (CAPTION: spare rolls of toilet paper)

CAPTION: the woman wearing red is looking at a pool in front of a brown building
FEEDBACKS:["A woman wearing red is standing with her back to a pool, not looking at it.", "The building is white not brown.", NaN]
MISALIGNMENT: The woman is standing with her back to a pool (CONTRADICTION: woman standing with her back to a pool), as described in the caption (CAPTION: woman looking at a pool). The building is white (CONTRADICTION: white building), not brown (CAPTION: brown building)

CAPTION: A yellow and green fire hydrant in Canada.
FEEDBACKS:["There is an all green fire hydrant, whose location could be anywhere, but isn't specifically Canadian.", "The hydrant is only green, not yellow and green.", "The fire hydrant is green and black, not green and yellow."]
MISALIGNMENT: The fire hydrant is only green (CONTRADICTION: green fire hydrant), not yellow and green (CAPTION: yellow and green fire hydrant).
"""

SAMPLETEMPLATE = """CAPTION: <caption>
FEEDBACKS: <feedback>
MISALIGNMENT:
"""


==> sec/9_acknowledgments.tex <==
\subsubsection*{Acknowledgments}
We express our gratitude to Amir Globerson, Jay Tenenbaum, and Shlomi Fruchter for their valuable feedback on earlier versions of the manuscript. We thank Jialin Wu and Sebastian Goodman for their help. This research was supported in part by the Israel Science Foundation (grants no. 2492/20, 3441/21 and 3611/21), Len Blavatnik and the Blavatnik family foundation.

==> tables/OOD.tex <==
\begin{table*}[!t]
\centering
% \caption{Overview of the Out Of Distribution evaluation featuring model performance over text-image pairs generated/captioned from multiple sources.}
\caption{Qualitative analysis of out-of-distribution results: Showcasing image-text pairs generated by six different text-to-image models alongside the corresponding textual and visual feedback as predicted by the PaLI 55B ft. \trainset model. }
\scriptsize % Even smaller font size
\setlength{\tabcolsep}{3pt} % Reduce space between columns
\renewcommand{\arraystretch}{1} % Reduce space between rows
\begin{tabularx}{\textwidth}{@{} *{7}{>{\centering\arraybackslash}X} @{}} % Adjusted for 7 columns with X type for auto-width
\toprule
\textbf{Source} & \textbf{SD XL} & \textbf{SD 2.1} & \textbf{Adobe Firefly} & \textbf{Attend-and-excite} \\
\midrule
\textbf{Input Prompt} & Two colleagues, one with a blue umbrella and the other without an umbrella, walking in the snow. & A young couple sharing pizza in a park, the man holds a slice in his hand. & A blue cat is sitting next to a green dog &  A red bench and a yellow clock \\
\midrule
\textbf{Generated Image} & \includegraphics[width=3.5cm,height=3.5cm]{images/OOD_no_bbox/split2_no_bbox_38.png}  & \includegraphics[width=3.5cm,height=3.5cm]{images/OOD_no_bbox/split2_no_bbox_207.png} & \includegraphics[width=3.5cm,height=2.5cm]{images/OOD_no_bbox/split1_no_bbox_128.png} & \includegraphics[width=3.5cm,height=3.5cm]{images/OOD_no_bbox/split1_no_bbox_53.png} \\
\midrule
\textbf{Predicted Textual \& Visual Feedback} & \includegraphics[width=3.5cm,height=3.5cm]{images/ood_bbox/split2_38.png} & \includegraphics[width=3.5cm,height=3.5cm]{images/ood_bbox/split2_207.png} & \includegraphics[width=3.5cm,height=3.5cm]{images/ood_bbox/split1_128.png} & \includegraphics[width=3.5cm,height=3.5cm]{images/ood_bbox/split1_53.png} \\
& One of the colleagues is holding an umbrella, not without an umbrella & The man is holding a whole pizza, not a slice & The cat is sitting next to a green cat, not a green dog &  The clock is black and white, not yellow \\
\bottomrule
\end{tabularx}
\label{table:OOD}
    
\end{table*}


==> tables/results_main_backup.tex <==

\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccc}
        \toprule
        & \multicolumn{2}{c}{\makecell{Feedback\\ BERTScore}} & \multicolumn{2}{c}{\makecell{Textual Misalignment\\BERTScore}} & \multicolumn{2}{c}{\makecell{Visual Misalignment\\BERTScore}} & \multicolumn{1}{c}{Precision@0.75} & \multicolumn{1}{c}{Recall@0.75}  & \multicolumn{1}{c}{Binary Acc.} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10}
        Model / Split & Test & Val & Test & Val & Test & Val & Test & Test & Test\\
        \midrule
        PaLI 5B
            & 0.463 & 0.641 & 0.496 & 0.615 & 0.580 & \textbf{0.622} & 0.401 &  0.570 & 0.514 \\
        InstructBLIP (FlanT5\textsubscript{XL}) \cite{instructblip}
            & 0.507 & 0.509 & 0.654 & 0.595 & 0.629 & 0.565 & 0.449 & 0.518 & 0.736 \\
        mPLUG-Owl (LLaMa-7B-ft) \cite{ye2023mplugowl}
            & 0.645 & 0.619 & 0.567 & 0.598 & 0.545 & 0.592 & 0.343 & \textbf{0.596} & 0.504 \\
        MiniGPT-v2 (7B-ft) \cite{chen2023minigptv2}
            & 0.647 & 0.636 & 0.616 & 0.580 & 0.613 & 0.580 & 0.417 & 0.467 & 0.676 \\
        LLaVa-1.5 (Vicuna-7b) \cite{liu2023improvedllava}
            & 0.692 & 0.663 & 0.549 & 0.573 & 0.534 & 0.570 & 0.343 & 0.590 & 0.717 \\
        \midrule
        PaLI 5B ft. Multitask
            & 0.837 & \textbf{0.926} & 0.779 & \textbf{0.882} & 0.691 & 0.456 & 0.634 & 0.397 & 0.752 \\
        PaLI 17B ft. Multitask 
            & 0.836 & 0.901 & \textbf{0.797} & 0.838 & \textbf{0.714} & 0.434 & 0.480 & 0.280 & 0.770 \\
        PaLI 55B ft. Multitask
            & \textbf{0.845} & 0.916 & 0.777 & 0.868 & 0.690 & 0.454 & \textbf{0.656} & 0.391 & \textbf{0.787} \\
        \bottomrule
    \end{tabular}}
    \caption{Comparative performance of vision-language models on the \testset Benchmark, highlighting the advancements in feedback generation achieved by fine-tuned PaLI models. Precision/Recall@0.75 signify the use of an IoU threshold of 0.75.
    \danix{typeset best result in each column in boldface.}
    }
    \label{tab:main_results_backup}
\end{table*}



